Algorithmic Threshold for Multi-Species Spherical Spin Glasses

We study efficient optimization of the Hamiltonians of multi-species spherical spin glasses. Our results characterize the maximum value attained by algorithms that are suitably Lipschitz with respect to the disorder through a variational principle that we study in detail. We rely on the branching overlap gap property introduced in our previous work and develop a new method to establish it that does not require the interpolation method. Consequently our results apply even for models with non-convex covariance, where the Parisi formula for the true ground state remains open. As a special case, we obtain the algorithmic threshold for all single-species spherical spin glasses, which was previously known only for even models. We also obtain closed-form formulas for pure models which coincide with the $E_{\infty}$ value previously determined by the Kac-Rice formula.

==> final-tex/5-amp.tex <==
\section{Approximate Message Passing}
\label{sec:amp}


\mscomment{
This section will be split off. Update things after writing augmented AMP in the appendix.
}

\mscomment{
Augmented state evolution can be used to analyze pairs of outputs by just doing both in the same sequence, so the suggestion of \cite{alaoui2020algorithmic} actually works now. It is worth commenting that for isoperimetric randomness, one can do AMP algorithms along a rooted tree of finite depth but exponential breadth.
}


In this section we prove Theorem~\ref{thm:main-alg} by exhibiting an approximate message passing (AMP) algorithm.
Throughout this section, Assumption~\ref{as:nondegenerate} on non-degeneracy of $\xi$ will be enforced. 
This is without loss of generality since one can always increase the quadratic and cubic coefficients $\gamma_{s,s'}, \gamma_{s,s',s''}$ by small constants and invoke continuity of $\ALG$.


As in \cite{alaoui2022algorithmic,sellke2021optimizing}, our algorithm has two phases. The first phase identifies the root of the ``algorithmic ultrametric tree'' and the second descends it in small orthogonal steps.
The structure of the first phase is similar to the original AMP algorithm of \cite{bolthausen2014iterative} for the SK model at high-temperature, while the latter \emph{incremental} AMP technique was introduced in \cite{mon18}. 




\subsection{Review of Approximate Message Passing}

Here we recall the class of approximate message passing algorithms, specialized to our setting of interest. We initialize AMP with a deterministic vector $\bw^0$  with coordinates
\begin{equation}
\label{eq:AMP-init-concrete}
    w^0_i = C_{s(i)}
\end{equation}
depending only on the species.
Let $f_{t,s}:\bbR^{t+1}\to\bbR$ be a Lipschitz function for each $(t,s)\in \bbZ_{\geq 0}\times \sS$. For $(\bw^0,\bw^1,\dots,\bw^t)\in\bbR^{N\times (t+1)}$, let 
$f_{t}(\bw^0,\bw^1,\dots,\bw^t)\in\bbR^N$ be given by
\[
    f_{t}(\bw^0,\bw^1,\dots,\bw^t)_i
    =
    f_{t,s(i)}(w^1_i,\dots,w^t_i),\quad i\in [N].
\]
We generate subsequent iterates through recursions of the form, where $\ONS_t$ is known as the \emph{Onsager correction term}:
\begin{align}
\label{eq:AMP-body}
    \bw^{t+1}
    &=
    \nabla H_N(\bm^t)
    -
    \ONS_t
    ;
    \\
\nonumber
    \bm^t
    &=
    f_{t}(\bw^0,\bw^1,\dots,\bw^t);
    \\
\label{eq:ONS-body}
    \ONS_t
    &=
    \sum_{t'\leq t}
    d_{t,t'}
    \diamond
    f_{t'-1}(\bw^1,\dots,\bw^{t'-1});
    \\
\label{eq:dts-def}
    d_{t,t',s}
    &=
    \sum_{s'\in\sS}
    \partial_{x_{s'}}
    \xi^s
    \lt(
    \lt(
    \bbE[M^t_{s''} M^{t'-1}_{s''}]\rt)_{s''\in\sS}
    \rt)
    \cdot
    \bbE
    \lt[
    \partial_{X^{t'}_{s'}}f_{t,s'}(X^0_{s'},\dots,X^t_{s'})
    \rt]
    .
\end{align}
Here $W^t_s,M^t_s$ are defined as follows. $W^0_s=C_s$ and the variables
$(\wt W^t_s)_{(t,s)\in \bbZ_{\geq 1}\times \sS}$ form a centered Gaussian process with covariance defined recursively by
\begin{equation}
\label{eq:state-evolution-basic}
\begin{aligned}
    \bbE[\wt W^{t+1}_s \wt W^{t'+1}_{s}]
    &=
    \xi^s\lt(\bbE[f_{t,s}(W^0_s,\dots,W^{t}_s)f_{t',s}(W^0_s,\dots,W^{t'}_s)]\rt),
    \\
    W^t_s
    &=
    \wt W^t_s+h_s;
    \\
    M^t_s
    &=
    f_{t,s}(W^0_s,\dots,W^t_s)
\end{aligned}
\end{equation}
and $\bbE[\wt W^{t+1}_{s} \wt W^{t'+1}_{s'}]=0$ if $s\neq s'$ (i.e. different species are independent). 


The following \emph{state evolution} characterizes the behavior of the above iterates. It states that for each $s\in\sS$, when $i\in \cI_s$ is uniformly random the sequence of coordinates $(w^1_i,w^2_i,\dots,w^t_i)$ has the same law as $(W^1_s,\dots,W^t_s)$. 


\begin{proposition}
\label{prop:state_evolution}
For any pseudo-Lipschitz function $\psi$ and $\ell\in\bbZ_{\geq 0}$, $s\in\sS$,
\begin{equation}
\label{eq:SE-body}
    \plim_{N\to\infty}\frac{1}{N_s}
    \sum_{i\in\cI_s}
    \psi(\bw^0_i,\dots,\bw^{\ell}_i)
    =
    \bbE
    [
    \psi(W^0_s,\dots,W^{\ell}_s)
    ]
    .
\end{equation}
\end{proposition}


This proposition allows us to read off normalized inner products of the AMP iterates, since e.g.
\[
    \langle \bw^k,\bw^{\ell}\rangle_N
    \simeq
    \sum_{s\in\sS}
    \lambda_s
    \bbE[W^k_s W^{\ell}_s].
\]



Proposition~\ref{prop:state_evolution} is proved in Appendix~\ref{sec:ProofSE}. For random matrices (i.e. the case of quadratic $H$) there is a considerable literature establishing state evolution in many settings beginning with \cite{bolthausen2014iterative,BM-MPCS-2011} and later \cite{bayati2015universality,berthier2019state,chen2020universality,fan2020approximate,dudeja2022universality} (see also \cite{feng2022unifying} for a survey of many statistical applications). The generalization to tensors was introduced in \cite{richard2014statistical} and proved in \cite{ams20}, whose approach we follow. 






\subsection{Stage $\I$: Finding the Root of the Ultrametric Tree}


Our goal in this subsection will be to compute a vector $\bm^{\ol}$ satisfying
\[
    \vR(\bm^{\ol},\bm^{\ol})\approx\Phi(q_0)
\]  
and with the correct energy value (as stated in Lemma~\ref{lem:sphereenergy} below). 




We take as given an maximizer $(p,\Phi;q_0)$ to $\bbA$ with associated transition point $q_1$. Recall this means there is a unique-up-to-scaling vector $v\in\mathbb R_{\geq 0}^{\sS}$ such that
\begin{equation}
\label{eq:v-equation}
    \lt(\xi^s(\Phi(q_1))+h_s^2\rt)v_s=
    \sum_{s'\in\sS}
    \partial_{x_s}\xi^{s'}
    (\Phi(q_1))
    \,
    \Phi_s(q_1)v_{s'}.
\end{equation}
We use the initialization
\[
    w^0_i = \sqrt{\xi^s(\Phi(q_1))+h_s^2},\quad i\in \cI_s.
\]
Define the vector $\va\in\mathbb R^{\sS}$ by 
\[
    a_s=
    \sqrt{\frac{\Phi_s(q_1)}{\xi^s(\Phi(q_1))+h_s^2}}
    =\sqrt{\frac{v_s}
    {\sum_{s'\in\sS} 
    \partial_{x_s} \xi^{s'}(\Phi(q_1))v_{s'}}}.
\]
Subsequent iterates are defined via the following recursion.
\begin{align}
\label{eq:RSsphere}
  \bw^{k+1}
  &=
  \nabla H_N(\bm^k)
  -
  \lt(\va\odot
    \zeta\big(\vR(\bm^k,\bm^{k-1})\big)
  \rt)
  \diamond
  \bm^{k-1}
  \\
\nonumber
  &=
  \bh
  +
  \nabla \wtH_N(\bm^k)
  -
  \lt(\va\odot
    \zeta\big(\vR(\bm^k,\bm^{k-1})\big)
  \rt)
  \diamond
  \bm^{k-1};
  \\
\label{eq:mk-def}
  \bm^k
  &=
  \va\diamond \bw^k
\\
\label{eq:zeta-defn}
    \zeta^s(\vx)
    &\equiv
    \sum_{s'\in \sS}
    \partial_{x_{s'}} \xi^s
    (\vx)
    .
\end{align}
The last term in \eqref{eq:RSsphere} comes from specializing the formula \eqref{eq:ONS-body} for the Onsager term.


Next recalling \eqref{eq:state-evolution-basic}, let $(W^j_s,M^j_s)_{j\geq 0,s\in\sS}$ be the state evolution limit of the coordinates of 
\[
    (\bw^{0},\bm^{0},\dots,\bw^k,\bm^k)
\]
as $N\to\infty$. Concretely, each $W^j_s$ is Gaussian with mean $h_s$ and 
\[
    M^{j}_s=\sqrt{\frac{\Phi_s(q_1)}{\xi^s(\Phi(q_1))+h_s^2}
    }
    \cdot 
    W^j_s,
    \quad
    j\geq 0,~
    s\in\sS.
\]
We next determine the covariance structure of the Gaussians $\wt W^j_s$. Define the (deterministic) $\mathbb R_{\geq 0}^{\sS}$-valued sequence $(R^0,R^1,\dots)$ of asymptotic overlaps recursively by $R^0=0$ and 
\begin{equation}
\label{eq:overlap-recursion-AMP}
    R^{k+1}_s=\alpha_s(R^k)=\lt(\xi^s(R^k)+h_s^2\rt)\cdot \lt(\frac{\Phi_s(q_1)}{\xi^s(\Phi(q_1))+h_s^2}\rt),\quad
    k\geq 0,s\in \sS.
\end{equation}



\begin{lemma}
\label{lem:RSconverge}
For integers $0\leq j<k$, the following equalities hold (the first in distribution):
\begin{align} 
\label{eq:id1.0}
    W^j_s&\stackrel{d}{=} h_s+Z\sqrt{\xi^s(\Phi(q_1))},\quad Z\sim \cN(0,1)\\
\label{eq:id2.0}
    \mathbb E[\wt W^j_s \wt W^k_s]&=\xi^s(R^j)\\
\label{eq:id3.0}
    \mathbb E[(M^j_s)^2]&=\Phi_s(q_1)\\
\label{eq:id4.0}
    \mathbb E[M^j_s M^k_s]&=R^{j+1}_s.
\end{align}
\end{lemma}



\begin{proof}
We proceed by induction on $j$, first showing \eqref{eq:id1.0} and \eqref{eq:id3.0} together. As a base case, \eqref{eq:id1.0} holds for $j=0$ by initialization. For the inductive step, assume first that \eqref{eq:id1.0} holds for $j$. Then by the definition \eqref{eq:mk-def},
\begin{align*}
  \mathbb E\lt[(M^j_s)^2\rt]&=
  \lt(\xi^s(\Phi(q_1))+h_s^2\rt)\cdot \lt(\frac{\Phi_s(q_1)}{\xi^s(\Phi(q_1))+h_s^2}\rt)
  \\
  &=\Phi_s(q_1)
\end{align*}
so that \eqref{eq:id1.0} implies \eqref{eq:id3.0} for each $j\geq 0$. On the other hand, state evolution directly implies that if \eqref{eq:id3.0} holds for $j$ then \eqref{eq:id1.0} holds for $j+1$. This establishes \eqref{eq:id1.0} and \eqref{eq:id3.0} for all $j\geq 0$.


We similarly show \eqref{eq:id2.0} and \eqref{eq:id4.0} together by induction, beginning with \eqref{eq:id2.0}. When $j=0$ it is clear because $\wt W^k_s$ is mean zero and independent of $\wt W^0_s$. 
Just as above, it follows from state evolution that \eqref{eq:id2.0} for $(j,k)$ implies \eqref{eq:id4.0} for $(j,k)$ which in turn implies \eqref{eq:id2.0} for $(j+1,k+1)$. Hence induction on $j$ proves \eqref{eq:id2.0} and \eqref{eq:id4.0} for all $(j,k)$.
\end{proof}


The next lemma is crucial and uses super-solvability of $\Phi(q_1)$.


\begin{lemma}
\label{lem:Rj-to-Phiq1}
    $\lim_{j\to\infty} R^j=\Phi(q_1).$
\end{lemma}


\begin{proof}
    First we observe that $\alpha$ is coordinate-wise strictly increasing in the sense that if $0\preceq x\prec y$ then $\alpha(x)\prec \alpha(y)$. 
    Moreover $\alpha(\vzero)\succ 0$ (assuming $\vh\neq 0$, else the result is trivial) and $\alpha(\Phi(q_1))=\Phi(q_1)$. Therefore $\oR=\lim_{j\to\infty} R^j$ exists, $\alpha(\oR)=\oR$, and
    \[
        \vzero\preceq \oR\preceq\Phi(q_1).
    \]
    It remains to show that the above forces $\oR=\Phi(q_1)$ to hold.
    
    
    Let $M\in\bbR^{\sS\times \sS}$ be the matrix with entries $M_{s,s'}=\deriv{t}\alpha_s'(\Phi(q_1)+te_{s'})|_{t=0}$ for $e_{s'}$ a standard basis vector. Then $M$ is the derivative matrix for $\alpha$ at $\Phi(q_1)$ in the sense that for any $u\in\bbR^{\sS}$,
    \[
        \deriv{t}\alpha'(\Phi(q_1)+tu)|_{t=0}=Mu.
    \]
    It is easy to see that all entries of $M$ are strictly positive, and that $Mv=v$ for $v$ solving \eqref{eq:v-equation}. By Perron-Frobenius theory, it follows that for any entry-wise non-negative vector $w\in\mathbb R_{\geq 0}^{\sS}$, we have
    \begin{equation}
    \label{eq:Mws} 
        (Mw)_s\leq w_s
    \end{equation}
    for some $s\in \sS$. Now suppose for sake of contradiction that $\oR\prec \Phi(q_1)$, let $w=\Phi(q_1)-\oR$, and choose $s^*\in\sS$ such that \eqref{eq:Mws} holds. Write $f(t)=\alpha_{s^*}(\Phi(q_1)+tw)$. Since $\alpha_{s^*}$ is a polynomial with non-negative coefficients and $\xi$ is non-degenerate, $f$ is strictly convex and strictly increasing on $[-1,0]$. Hence
    \begin{align*}
        \alpha_{s^*}(\oR)
        &= f(-1)
        \\
        &>
        f(0)-f'(0)
        \\
        &\geq
        \Phi_{s^*}(q_1)-(Mw)_{s^*}
        \\
        &\stackrel{\eqref{eq:Mws}}{\geq}
        \Phi_{s^*}(q_1)-w_{s^*}
        \\
        &=
        \oR_{s^*}.
    \end{align*}
    The first inequality above is strict, so we deduce that $\alpha(\oR)\neq\oR$ if $\oR\prec\Phi(q_1)$. This contradicts the definition of $\oR$. Therefore $\oR=\Phi(q_1)$, completing the proof.
\end{proof}


\begin{remark}
Super-solvability of $\Phi(q_1)$ is precisely the required condition for the above to go through. It is equivalent to the matrix $M=\alpha'$ above having Perron-Frobenius eigenvalue at most $1$. Indeed suppose that $\Phi(q_1)$ was chosen so that $\lambda_1(M)>1$. Then there exists $w\in\bbR_{>0}^{\sS}$ with $Mw\succ w$.
Letting $x=\Phi(q_1)-\eps w$ for small $\eps>0$, we find $\alpha(x)\prec x$.
Monotonicity implies that $\alpha$ maps the compact, convex set
\[
    K=\{y\in[0,1]^{\sS}~:~0\preceq y\preceq x\}
\]
into itself. By the Brouwer fixed point theorem, a fixed point of $\alpha$ strictly smaller than $\Phi(q_1)$ exists whenever $\Phi(q_1)$ is strictly subsolvable.
\end{remark}


We finish our analysis of the first AMP phase by computing the asymptotic energy it achieves. As expected, the resulting value agrees with the first term in the formula \eqref{eq:alg-for-optimizer} for $\ALG$.
%
\begin{lemma}
\label{lem:sphereenergy}
\[
  \lim_{k\to\infty} \plim_{N\to\infty}\frac{H_N(\bm^k)}{N}
  = 
    \sum_{s\in \sS}
    \lambda_s
      \sqrt{
      \Phi_s(q_1)
      \cdot
      \lt(h_s^2+\xi^s(\Phi(q_1))\rt)
      }
    \,.
\]
\end{lemma}

\begin{proof}

We use the identity
\begin{equation}
  \frac{H_N(\bm^k)}{N}=\big\langle \bh,\bm^k\rangle_N+\int_0^1 \langle \bm^k,\nabla \widetilde H_N(t\bm^k)\big\rangle_N \de t
\end{equation}
and interchange the limit in probability with the integral. To compute $\plim_{N\to\infty}\langle \bm^k,\nabla \widetilde H_N(t\bm^k)\rangle$ we introduce an auxiliary AMP step 
\[
    \by^{k+1}=\nabla \widetilde H_N(t\bm^k)-
    t\cdot
    \lt(\va\odot
    \zeta\big(
        t\cdot \vR(\bm^k,\bm^{k-1})
    \big)
    \rt)
    \diamond
    \bm^{k-1}
\] 
which depends implicitly on $t\in [0,1]$.
Rearranging yields
\begin{align*}
  \vR(\bm^k,\nabla \widetilde H_N(t\bm^k)) 
  &= 
  \vR(\bm^k,\by^{k+1})
  +
  t\cdot
  \lt(
  \vR(\bm^k,\bm^{k-1} )
  \odot \va
  \odot 
  \zeta(t\cdot \vR(\bm^k,\bm^{k-1}) )
  \rt)  
  \\
  &\simeq   
  \vR( \bm^k,\by^{k+1})
  +
  t\cdot
  \lt(
  \vR^k
  \odot \va
  \odot 
  \zeta(t\cdot \vR^k )
  \rt)  
  .
\end{align*}

For the first term, Gaussian integration by parts with $g_s(x)=(x+h_s)a_s$ yields
\begin{align*}
    R_s(\bm^k,\by^{k+1})
    &=
  \mathbb E[g_s(W^k)Y^{k+1}_s]
  \\
  &=
  \mathbb E[g_s'(W^k)]
  \cdot
  \mathbb E[W^k_s Y^{k+1}_s]
  \\
  &= 
  a_s
  \cdot 
  \xi^s(t R^k)
  .
\end{align*}
Integrating with respect to $t$, we find
\begin{align*} 
  \int_0^1 \langle \bm^k,\nabla \widetilde H_N(t\bm^k)\rangle_N \de t
  &\simeq 
  \sum_{s\in\sS}
  \lambda_s 
  \int_0^1
  R_s(\bm^k,\nabla \widetilde H_N(t\bm^k))
  \de t
  \\
  &\simeq
  \sum_{s\in\sS}
  \lambda_s
  a_s
  \int_0^1
  \xi^s(t\cdot \vR^k)
  +
  t R^k_s \zeta^s(t\cdot \vR^k)
  \de t 
  \\
  &=
  \sum_{s\in\sS}
  \lambda_s
  a_s
  \int_0^1
  \frac{\de ~}{\de t}
  \lt(t\cdot \xi^s(t\cdot \vR^k)\rt)
  \de t
  \\
  &=
  \sum_{s\in\sS}
  \lambda_s a_s \xi^s(\vR^k).
\end{align*}
Finally the external field $\bh$ gives energy contribution
\[
  \langle \bh, \bm^k\rangle_N 
  \simeq 
  \sum_{s\in\sS}
  \lambda_s
  h_s\bbE[M^k_s]
  =
  \sum_{s\in\sS}
  \lambda_s
  a_s
  h_s^2.
\]
Since $\lim_{k\to\infty} R^{k}=\Phi(q_1)$ by Lemma~\ref{lem:Rj-to-Phiq1}, we conclude
\begin{align*}
  \lim_{k\to\infty} \plim_{N\to\infty}\frac{H_N(\bm^k)}{N}
  &= 
  \sum_{s\in\sS}
  \lambda_s
  a_s\big(h_s^2 + \xi^s(\Phi(q_1))\big)
  \\
  &=
  \sum_{s\in\sS}
  \lambda_s
  \sqrt{
    \Phi_s(q_1)
  \cdot
  \lt(h_s^2+\xi^s(\Phi(q_1))\rt)
  }
  .
\end{align*}
\end{proof}


\subsection{Stage $\II$: Incremental Approximate Message Passing}


We now turn to the second phase which uses incremental approximate message passing. Choose a large constant $\ul$ and set
\begin{align*}
    \eps_s
    &=
    \sqrt{\frac{\Phi(q_0)_s}{R^{\ul}_s}}
    -1,
    \\
    \bn^{\ul}
    &=
    (1+\eps)
    \diamond 
    \bm^{\ul}
\end{align*}
so that 
\[
    \vR(\bn^{\ul},\bn^{\ul})\simeq \Phi(q_1).
\]
The point $\bn^{\ul}$ will be the ``root'' of our IAMP algorithm.\footnote{If $\vh=0$, one can instead set $n^{\ul}_i=\sqrt{\Phi_{s(i)}(\delta)}\diamond \bg$ for $\bg\sim\cN(0,I_N)$ and use the same algorithm with $q_0=0$.} We fix a small constant $\delta>0$ and consider the sequence
\[
    q^{\delta}_{\ell} 
    =
    q_1
    +
    \ell\delta,\quad \ell\geq 0.
\]
Moreover we set $\ol=\max\{\ell\in\bbZ_+~:~q_{\ell}^{\delta}\leq 1-2\delta\}.$
We also define for $s\in\sS$ and $\ul\leq \ell\leq \ol$ the constants
\begin{equation}
\label{eq:u-def}
    u_{\ell,s}^{\delta}
    =
    \sqrt{
    \frac{\Phi_s(q^{\delta}_{\ell+1})-\Phi_s(q^{\delta}_{\ell})}
    {
    \xi^s(\Phi(q_{\ell+1}^{\delta}))
    -
    \xi^s(\Phi(q_{\ell}^{\delta}))
    }
    }
    .
\end{equation}



Set $\bz^{\ul}=\wt\bw^{\ul}=\bw^{\ul}-\bh$.
So far, we have defined $(\bw^{\ul},\bz^{\ul},\bn^{\ul})$. We turn to inductively defining the triples $(\bw^{\ell},\bz^{\ell},\bn^{\ell})$ for $\ul\leq\ell\leq\ol$. First, the values $(\bz^{\ell})_{\ell\geq \ul}$ are defined as AMP iterates via
\begin{equation}
\label{eq:general_amp}
\begin{aligned}
    \bz^{\ell+1} 
    &= 
    \nabla \widetilde H_N(f_{\ell}(\bz^{\ul},\cdots,\bz^\ell)) - \sum_{j=0}^\ell d_{\ell, j}\diamond f_{j-1}(\bz^{\ul},\cdots,\bz^{j-1})
    .
\end{aligned}
\end{equation}
The Onsager coefficients $d_{\ell,j}$ are given by \eqref{eq:dts-def} and will not appear explicitly in any calculations.
Here the variables $Z^k$ are the state evolution limits. To complete the definition of the iteration \eqref{eq:general_amp}, for $s(i)=s$ and $\ell\geq \ul$ we set
\[
    f_{\ell,s}(z^{\ul}_i,\dots,z^{\ell}_i)
    =
    n^{\ell}_i,
\]
where
\begin{equation}
\label{eq:IAMP}
    \bn^{\ell+1} 
    =
    \bn^{\ell}+ 
    u_{\ell}^{\delta}
    \diamond
    \lt(\bz^{\ell+1}-\bz^{\ell}
    \rt).
\end{equation} 
Finally the algorithm $\cA$ outputs
\begin{equation}
\label{eq:round-final-output}
    \cA(H_N)
    =
    R(\bn^{\ol},\bn^{\ol})^{-1/2}\diamond \bn^{\ol}
    \in\cB_N
\end{equation}
where the power $-1/2$ is taken entry-wise.

The state evolution limits are described by time-changed Brownian motions with total variance $\Phi_s(q^{\delta}_{\ell})$ in species $s$ after iteration $\ell$. This is made precise below.

\begin{lemma}
\label{lem:BMlimit}
Fix $s\in\sS$. The sequence $(Z^{\delta}_{\ul,s},Z^{\delta}_{\ul+1,s},\dots)$ is a Gaussian process satisfying
\begin{align} 
\label{eq:BM1}
    \mathbb E[(Z^{\delta}_{\ell+1,s}-Z^{\delta}_{\ell,s})Z^{\delta}_{j,s}]
    &=
    0,\quad \text{for all }\ul+1\leq j\leq \ell
    \\
\label{eq:BM2}
    \mathbb E\big[
    (Z^{\delta}_{\ell+1,s}-Z^{\delta}_{\ell,s})^2
    \big]
    &=
    \xi^s(\Phi(q_{\ell+1}^{\delta}))
    -
    \xi^s(\Phi(q_{\ell}^{\delta}))
    \\
\label{eq:BM3}
    \mathbb E[Z^{\delta}_{\ell,s}Z^{\delta}_{j,s}]
    &=
    \xi^s(\Phi(q_{j\wedge \ell}^{\delta}))
    \\
\label{eq:BM4}
    \mathbb E[N^{\delta}_{\ell,s}N^{\delta}_{j,s}]
    &=
    \Phi_s(q^{\delta}_{j\wedge \ell})
    .
\end{align}
\end{lemma}


\begin{proof}
The fact that $(Z^{\delta}_{\ul,s},Z^{\delta}_{\ul+1,s},\dots)$ is a Gaussian process is a general fact about state evolution. We proceed by induction on $\ell\geq \ul$; in fact the proof is very similar to \cite[Section 8]{sellke2021optimizing} so we give only the main points. For the base case, the main computation is that 
\begin{align*}
    \bbE\big[\big(Z^{\delta}_{\ul+1,s}-Z^{\delta}_{\ul,s}\big)Z^{\delta}_{\ul,s}\big]
    &=
    \xi^s\lt(\bbE[N^{\delta}_{\ul,s}M^{\ul-1}_s]\rt)
    -
    \xi^s\lt(\bbE[M^{\ul-1}_{s}M^{\ul-1}_s]\rt)
    \\
    &=
    \xi^s\lt((1+\eps_s)\bbE[M^{\ul}_s M^{\ul-1}_s]\rt)-\xi^s(\Phi(q_1))
    \\
    &=
    \xi^s(\Phi(q_1))-\xi^s(\Phi(q_1))
    \\
    &=
    0.
\end{align*}
For inductive steps, we always have by state evolution
\[
    \bbE[Z^{\delta}_{\ell+1,s}Z^{\delta}_{j+1,s}]
    \simeq
    \xi^s\big(\vR(\bn^{\ell},\bn^{j})\big).
\]
It follows by the inductive hypothesis of \eqref{eq:BM1} that for $j\leq \ell$,
\begin{align*}
    R_s(\bn^{\ell},\bn^{j})
    &=
    R_s(\bn^{\ul},\bn^{\ul})
    +
    \sum_{k=\ul}^{j-1}
    (u_k^{\delta})^2
    R_s(\bz^{k+1}-\bz^k,\bz^{k+1}-\bz^k)
    \\
    &=
     R_s(\bn^{\ul},\bn^{\ul})
     +
     \sum_{k=\ul}^{j-1}
     (u_k^{\delta})^2
     \lt(
      \xi^s(\Phi(q_{k+1}^{\delta}))
    -
    \xi^s(\Phi(q_{k}^{\delta}))
    \rt)
    \\
    &=
    \Phi_s(q_1)
    +
    \sum_{k=\ul}^{j-1}
    \Big(
    \Phi_s(q^{\delta}_{k+1})
    -
    \Phi_s(q^{\delta}_{k})
    \Big)
    \\
    &=
    \Phi_s(q^{\delta}_j).
\end{align*}
Plugging into the above yields that for $j\leq \ell$,
\[
    \bbE[Z^{\delta}_{\ell+1,s}Z^{\delta}_{j+1,s}]
    =
    \xi^s(\Phi(q^{\delta}_j)).
\]  
This depends only on $\min(j,\ell)$, so \eqref{eq:BM1} follows. The others are proved by similar computations.
\end{proof}


Equation~\eqref{eq:BM4} implies that $\vR(\bn^{\delta}_{\ell},\bn^{\delta}_{j})\simeq \Phi(q^{\delta}_{\ell\wedge j})$, which exactly corresponds to the previous sections of the paper. In particular it implies that the final iterate $\bn^{\delta}_{\ol}$ satisfies
\begin{equation}
\label{eq:final-overlap-alg}
    (1-O(\delta))\cdot\vone\preceq \vR(\bn^{\delta}_{\ol},\bn^{\delta}_{\ol})\preceq \vone
\end{equation}
so the rounding step \eqref{eq:round-final-output} causes only an $O(\delta)$ change in the Hamiltonian value. Finally we compute in Lemma~\ref{lem:iampenergy} below the energy gain from the second phase, which matches the second term in \eqref{eq:alg-for-optimizer}. 


\begin{lemma}
\label{lem:iampenergy}
\begin{equation}
    \label{eq:iampenergy}
    \lim_{\ul\to\infty}
    \plim_{N \to \infty}
    \frac{H_{N}\lt(\bn^{\ol}\rt)-H_{N}\lt(\bn^{\ul}\rt)}{N} 
    = 
    \sum_{s\in\sS}
  \lambda_s
  \int_{q_1}^{1} 
    \sqrt{\Phi'_s(t) (\xi^s \circ \Phi)'(t)}
    \,
    \de t
\end{equation}
\end{lemma}



\begin{proof}
Recall that $\delta=\delta(\ul)\to 0$ as $\ul\to\infty$, which we will implicitly use throughout the proof. Observe also that $\langle h,\bn^{\ol}-\bn^{\ul}\rangle_N\simeq 0$ because the values $(N_{\ell,s}^{\delta})_{\ell\geq\ul}$ form a martingale sequence for each $s\in\sS$. 
Therefore it suffices to compute the in-probability limit of $\frac{\widetilde{H}_{N}\lt(\bn^{\ol}\rt)-\widetilde{H}_{N}\lt(\bn^{\ul}\rt)}{N}$. The key is to write 
\[
    \frac{\widetilde{H}_{N}\lt(\bn^{\ol}\rt)-\widetilde{H}_{N}\lt(\bn^{\ul}\rt)}{N}=\sum_{\ell=\ul}^{\ol-1}\frac{\widetilde{H}_{N}\lt(\bn^{\ell+1}\rt)-\widetilde{H}_{N}\lt(\bn^{\ell}\rt)}{N}
\]
and use a Taylor series approximation for each term. In particular for $F\in C^3(\mathbb R;\bbR)$, applying Taylor's approximation theorem twice yields
\begin{align*}
    F(1)-F(0)
    &=
    F'(0)+\frac{1}{2}F''(0)+O(\sup_{a\in [0,1]}|F'''(a)|)
    \\
    &= 
    F'(0)+\frac{1}{2}(F'(1)-F'(0))+O(\sup_{a\in [0,1]}|F'''(a)|)
    \\
    &=
    \frac{1}{2}(F'(1)+F'(0))+O(\sup_{a\in [0,1]}|F'''(a)|) .
\end{align*}

Assuming $\sup_{\ell}\frac{\|\bn^{\ell}\|}
{\sqrt{N}}\leq 1$, which holds with probability $1-o_N(1)$ by state evolution and the definition of $\ol$, we apply this estimate with 
\[
    F(a)=\widetilde{H}_N\lt((1-a)\bn^{\ell}+a\bn^{\ell+1}\rt).
\]
The result is:
\begin{align*}
    \lt|
    \widetilde{H}_{N}
    \lt(\bn^{\ell+1}\rt)-\widetilde{H}_{N}\lt(\bn^{\ell}\rt) -\frac{1}{2}\lt\langle \nabla \widetilde{H}_N(\bn^{\ell})+\nabla \widetilde{H}_N(\bn^{\ell+1}),\bn^{\ell+1}-\bn^{\ell}\rt\rangle \rt|
    &\leq 
    O\lt(
    \underline{C}N^{-1/2}
    \|\bn^{\ell+1}-\bn^{\ell}\|^3
    \rt)
    ;
    \\
    \underline{C}
    &=
    N^{1/2}
    \sup_{\|\bsig\|\leq \sqrt{N}}\lt\|\nabla^3 \widetilde{H}_N(\bsig)\rt\|_{\op}
    .
\end{align*}
Proposition~\ref{prop:gradients-bounded} implies that for deterministic constants $c,C$,
\[
    \bbP[\underline{C}\leq C]\geq 1-e^{-cN}.
\]
On the other hand for each $\ul\leq \ell\leq \ol-1$ we have
\begin{align*}
    \plim_{N\to\infty}\|\bn^{\ell+1}-\bn^{\ell}\|&=
    \sqrt{
    \sum_{s\in\sS}\lambda_s R_s(\bn^{\ell+1}-\bn^{\ell},\bn^{\ell+1}-\bn^{\ell})
    }
    \\
    &=
    \sqrt{
    \sum_{s\in\sS}\lambda_s
    \Phi_s(q^{\delta}_{\ell+1}-q^{\delta}_{\ell})
    }
    \\
    &=
    \sqrt{\delta N}.
\end{align*}
Summing and recalling that $\ol-\ul\leq \delta^{-1}$ yields the high-probability estimate
\begin{align*}
  \sum_{\ell=\ul}^{\ol-1}
  &
  \lt|
  \widetilde{H}_{N}\lt(\bn^{\ell+1}\rt)
  -
  \widetilde{H}_{N}\lt(\bn^{\ell}\rt) 
  -
  \frac{1}{2}\lt\langle  \nabla \widetilde{H}_N(\bn^{\ell})+\nabla \widetilde{H}_N(\bn^{\ell+1}),\bn^{\ell+1}-\bn^{\ell}\rt\rangle  
  \rt|
  \\ 
  &\leq 
  O(N^{-1/2})
  \cdot 
  \sum_{\ell=\ul}^{\ol-1} 
  \|\bn^{\ell+1}-\bn^{\ell}\|^3
  \\
  &\leq O(N\sqrt{\delta}).
\end{align*}
Because $\delta\to 0$ as $\ul\to\infty$, this term vanishes in the outer limit. It remains to prove
\[
  \lim_{\ul\to\infty}
  \plim_{N \to \infty}
  \sum_{\ell=\ul}^{\ol-1}
  \lt\langle 
  \nabla \widetilde{H}_N(\bn^{\ell})
  +
  \nabla \widetilde{H}_N(\bn^{\ell+1})
  ,
  \bn^{\ell+1}-\bn^{\ell}
  \rt\rangle_N  
  \stackrel{?}{=}
  2
  \sum_{s\in\sS}
  \lambda_s
  \int_{q_1}^{1} 
    \sqrt{\Phi'_s(t) (\xi^s \circ \Phi)'(t)}
  \de t.
\]
To establish this it suffices to show for each species $s\in\sS$ the equality
\begin{equation}
\label{eq:IAMP-energy-per-species}
  \lim_{\ul\to\infty}
  \plim_{N \to \infty}
  \sum_{\ell=\ul}^{\ol-1}
  R\lt(
  \nabla \widetilde{H}_N(\bn^{\ell})
  +
  \nabla \widetilde{H}_N(\bn^{\ell+1})
  ,
  \bn^{\ell+1}-\bn^{\ell}
  \rt)_s 
  \stackrel{?}{=}
  2
  \int_{q_1}^{1} 
    \sqrt{\Phi'_s(t) (\xi^s \circ \Phi)'(t)}
  \de t.
\end{equation}
This is what we do. Observe by \eqref{eq:general_amp} that:
%
\begin{equation}
\label{eq:amprearrange}
    \nabla \widetilde{H}_N(\bn^{\ell})
    =
    \bz^{\ell+1}- \sum_{j=0}^\ell d_{\ell, j}\diamond \bn^{j-1}.
%
\end{equation}
%
Passing to the limiting Gaussian process $(Z^{\delta}_k)_{k\in\mathbb Z^+}$ via state evolution,
\begin{align*}
  \plim_{N\to\infty}
  R\lt(\nabla \widetilde{H}_N(\bn^{\ell}),\bn^{\ell+1}-\bn^{\ell}\rt)_s
  &=
  \mathbb E\lt[ Z^{\delta}_{\ell+1,s}(N^{\delta}_{\ell+1,s}-N^{\delta}_{\ell,s})\rt]
  - 
  \sum_{j=0}^{\ell}
  d_{\ell,j,s}
  \mathbb E\lt[
  N^{\delta}_{j-1,s}(N^{\delta}_{\ell+1,s}-N^{\delta}_{\ell,s})
  \rt],
  \\
  \plim_{N\to\infty}
  R\lt(\nabla \widetilde{H}_N(\bn^{\ell+1}),\bn^{\ell+1}-\bn^{\ell}\rt)_s
  &=
  \mathbb E\lt[ Z^{\delta}_{\ell+2,s}(N^{\delta}_{\ell+1,s}-N^{\delta}_{\ell,s})\rt]
  - 
  \sum_{j=0}^{\ell+1} 
  d_{\ell+1,j,s}
  \mathbb E\lt[
  N^{\delta}_{j-1}(N^{\delta}_{\ell+1,s}-N^{\delta}_{\ell,s})
  \rt].
\end{align*}


As $(N^{\delta}_k)_{k\geq \mathbb Z^+}$ is a martingale process, it follows that the right-hand expectations all vanish. Similarly it holds that
\begin{align*}
  \mathbb E[Z_{\ell+2}^{\delta}(N_{\ell+1}^{\delta}-N_{\ell}^{\delta})]&=\mathbb E[Z_{\ell+1}^{\delta}(N_{\ell+1}^{\delta}-N_{\ell}^{\delta})]
  \\
  \mathbb E[Z_{\ell}^{\delta}(N_{\ell+1}^{\delta}-N_{\ell}^{\delta})]&=0.
\end{align*}
%
We conclude that
%
\begin{align*}
  \plim_{N\to\infty}
  R\lt(\nabla \widetilde{H}_N(\bn^{\ell})+\nabla \widetilde{H}_N(\bn^{\ell+1}),\bn^{\ell+1}-\bn^{\ell}\rt)_s
  &=
  2\,\mathbb E[
  (Z_{\ell+1,s}^{\delta}-Z^{\delta}_{\ell,s})(N_{\ell+1,s}^{\delta}-N_{\ell,s}^{\delta})
  ]
  \\
  &=
  2\,\mathbb E[u_{\ell,s}^{\delta}(Z^{\delta}_{\ell,s})(Z_{\ell+1,s}^{\delta}-Z^{\delta}_{\ell,s})^2]
  \\
  &=
  2\,\mathbb E[u_{\ell,s}^{\delta}(Z^{\delta}_{\ell,s})]
  \cdot
  \bbE[(Z_{\ell+1,s}^{\delta}-Z^{\delta}_{\ell,s})^2]
  \\
&=
  2\,\sqrt{
  \Big(
  \Phi_s(q^{\delta}_{\ell+1,s})-\Phi_s(q^{\delta}_{\ell,s})
  \Big)
  \cdot
    \Big(\xi^s(\Phi(q_{\ell+1}^{\delta}))-\xi^s(\Phi(q_{\ell}^{\delta}))
    \Big)
    }
    .
\end{align*}
In the second-to-last step we used the fact that $Z^{\delta}_{\ell,s}$ has independent increments, which follows from Lemma~\ref{lem:BMlimit}, while the last step used \eqref{eq:u-def} and \eqref{eq:BM2}.
Combining with Lemma~\ref{lem:ALG-from-continuum} implies \eqref{eq:IAMP-energy-per-species}.
\end{proof}


\begin{proof}[Proof of Theorem~\ref{thm:main-alg}]
We take $\cA$ as in \eqref{eq:round-final-output} for $\ul$ a large constant depending on $(\eps,\xi,h,\lambda)$. The fact that 
\begin{equation}
\label{eq:1-o1-prob-alg}
    \bbP[H_N(\cA(H_N))/N \geq \ALG-\eps/2]
    \ge 
    1-o_N(1)
\end{equation}
follows from combining Lemma~\ref{lem:sphereenergy}, Lemma~\ref{lem:iampenergy} and the fact that (recall \eqref{eq:final-overlap-alg}) 
\[
H_N(\cA(H_N))/N \simeq H_N(\bn^{\ul})/N+o_{\bbP}(1).
\]

Next, let $K_N\subseteq\sH_N$ be as in Proposition~\ref{prop:gradients-bounded}. We recall that $\bbP[H_N\in K_N]\geq 1-e^{-cN}$.
Exactly as in \cite[Theorem 10]{huang2021tight} it follows that there is a $C(\eps)$-Lipschitz function $\wt\cA:\sH_N\to\bbR$ such that $\wt\cA$ and $\cA$ agree on $K_N$.
Moreover \eqref{prop:gradients-bounded} and concentration of measure on Gaussian space imply that $H_N(\wt\cA(H_N))$ is $O(N^{1/2})$-sub-Gaussian. In light of \eqref{eq:1-o1-prob-alg} and since $\bbP[\wt\cA(H_N)=\cA(H_N)]\geq \bbP[H_N\in K_N]\geq 1-e^{-cN}$, we deduce that 
\[
    \bbP[H_N(\cA(H_N))/N \geq \ALG-\eps]
    \ge 
    1-e^{-cN}.
\]
This concludes the proof.
\end{proof}


\begin{remark}
    Analogously to \cite[Section 4]{sellke2021optimizing}, the second stage of our IAMP algorithm can be slightly modified to give a full ultrametric tree of outputs, whose pairwise overlaps are given by values of $\Phi$. More precisely, for any finite ultrametric space $X=(x_1,\dots,x_m)$ of diameter at most $1-q_1$, a branching variant of our algorithm outputs $(\bsig_1,\dots,\bsig_n)$ with
    \[
        \plim_{N\to\infty}
        \max_{1\leq i,j\leq m}\tnorm{
            \vR(\bsig_i,\bsig_j)
            - \Phi\big(1-d_X(x_i,x_j)\big)
        }_{\infty}=0.
    \]
    We omit the details of this extension.
\end{remark}



==> final-tex/6-parisi.tex <==
\section{Attaining the Ground State Energy in Full-RSB models}

\begin{align*}
    \CS(\zeta,\Phi,\vDelta)
    &= 
    \sum_{s\in \sS}
    \fr{\lambda_s}{2}
    \lt[
        \lambda_s^{-1}h_s^2\Delta_s(0)
        + 
        \int_0^1 \fr{\Phi'_s(q)}{\Delta_s(q)} + (\xi^s\circ \Phi)'(q)\Delta_s(q)~\de q
    \rt],\quad \text{where} \\
    \Delta_s(q) &= \Delta_s + \int_q^1 \zeta(t)\Phi'_s(t)~\de t.
\end{align*}

Suppose $\zeta$ is supported on $[q_1,1]$.
Note that because $\Delta_s(q)$ is constant for $q\in [0, q_1]$, $\CS(\zeta,\Phi,\vDelta) = \CS_1 + \CS_2$ for
\begin{align*}
    \CS_1 &= 
    \sum_{s\in \sS}
    \fr{\lambda_s}{2} 
    \lt[
        \fr{\Phi_s(q_1)}{\Delta_s(q_1)}
        +
        ((\xi^s \circ \Phi)(q) + h_s^2/\lambda_s) \Delta_s(q_1)
    \rt], \\
    \CS_2 &= 
    \sum_{s\in \sS}
    \fr{\lambda_s}{2} 
    \int_{q_1}^1
    \fr{\Phi'_s(q)}{\Delta_s(q)} + 
    (\xi^s\circ \Phi)'(q)\Delta_s(q)~\de q.
\end{align*}
Consider the perturbation
\[
    \tPhi_1(q) = \Phi_1(q) + \delta \psi(q)
\]
and $\tPhi_s(q) = \Phi_s(q)$ for $s\neq 1$.
Here $\psi$ is supported on $[q_1,1]$ with $\psi(q_1) = \psi(1)=0$.
Then 
\[
    \fr{\de}{\de \delta} (\xi^s \circ \Phi)(q) 
    = 
    (\psi \times \partial_1 \xi^s \circ \Phi)(q)
    =
    \fr{\lambda_s}{\lambda_1} (\psi \times \partial_s \xi^1 \circ \tPhi)(q),
    \qquad
    \fr{\de}{\de \delta} \Delta_1(q) 
    = 
    \int_q^1 \zeta(t) \psi'(t)~\de t
\]
and $\Delta_s(q)$ for $s\neq 1$ does not change under the perturbation.
Now,
\[
    F_1 
    \equiv
    \fr{\de}{\de \delta}
    2 \lambda_1^{-1} \CS_1 \Big|_{\delta=0} 
    = 
    \lt(
        -\fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
        +\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
    \rt) \lt(
        \int_{q_1}^1 \zeta(q) \psi'(q) ~\de q
    \rt).
\]
Moreover,
\[
    F_2 
    \equiv 
    \fr{\de}{\de \delta}
    2 \lambda_1^{-1} \CS_2 \Big|_{\delta=0} 
    = F_{2,1} + F_{2,2} + F_{2,3} 
\]
for
\begin{align*}
    F_{2,1}
    &= 
    \int_{q_1}^1 \fr{\psi'(q)}{\Delta_1(q)} ~\de q 
    = 
    -\int_{q_1}^1 
    \fr{\psi(q) \zeta(q) \Phi'_1(q)}{\Delta_1(q)^2} ~\de q \\
    F_{2,2}
    &= 
    \sum_{s\in \sS}
    \int_{q_1}^1 
    (\psi \times \partial_s\xi^1 \circ \Phi)'(q) 
    \Delta_s(q) ~\de q 
    =
    \sum_{s\in \sS} 
    \int_{q_1}^1 
    \psi(q) \zeta(q) (\partial_s \xi^1 \circ \Phi)(q) \Phi'_s(q) 
    ~\de q\\
    &=
    \int_{q_1}^1 
    \psi(q) \zeta(q) (\xi^1 \circ \Phi)'(q) 
    ~\de q \\
    F_{2,3}
    &= 
    \int_{q_1}^1 \lt(
        -\fr{\Phi'_1(q)}{\Delta_1(q)^2}
        + (\xi^1 \circ \Phi)'(q)
    \rt)\lt(
        \int_q^1 \zeta(t) \psi'(t) ~\de t
    \rt) ~\de q.
\end{align*}
Thus
\begin{align*}
    &\fr{\de}{\de \delta}
    \CS(\zeta,\tPhi,\vDelta) \Big|_{\delta = 0} \\
    &= \lt(
        -\fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
        +\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
    \rt) \lt(
        \int_{q_1}^1 \zeta(q) \psi'(q) ~\de t
    \rt) \\
    &\quad +
    \int_{q_1}^1 
    \lt(
        -\fr{\Phi'_1(q)}{\Delta_1(q)^2}
        + (\xi^1 \circ \Phi)'(q)
    \rt)\lt(
        \psi(q) \zeta(q) +
        \int_q^1 \zeta(t) \psi'(t) ~\de t
    \rt) ~\de q \\
    &= 
    \lt(
        \fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
        -\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
    \rt) \lt(
        \int_{q_1}^1 \psi(q) \zeta'(q) ~\de t
    \rt) \\
    &\quad +
    \int_{q_1}^1 
    \lt(
        \fr{\Phi'_1(q)}{\Delta_1(q)^2}
        - (\xi^1 \circ \Phi)'(q)
    \rt)\lt(
        \int_q^1 \psi(t) \zeta'(t) ~\de t
    \rt) ~\de q \\
    &= 
    \int_{q_1}^1 
    \psi(q) \zeta'(q) \lt(
        \fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
        -\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
        + 
        \int_{q_1}^q 
        \lt(
            \fr{\Phi'_1(t)}{\Delta_1(t)^2}
            - (\xi^1 \circ \Phi)'(t)
        \rt)
        ~\de t
    \rt) 
    ~\de q.
\end{align*}
Since $\zeta'>0$ on all of $[q_1,1]$, we have that
\[
    \fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
    -\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
    + 
    \int_{q_1}^q 
    \lt(
        \fr{\Phi'_1(t)}{\Delta_1(t)^2}
        - (\xi^1 \circ \Phi)'(t)
    \rt)
    ~\de t
    = 0
\]
almost everywhere on $[q_1,1]$.
This function is obviously continuous so it is zero everywhere on $[q_1,1]$.
Evaluating at $q=q_1$, we find
\[
    \Delta_1(q_1) 
    = 
    \sqrt{\fr{\Phi_1(q_1)}{(\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1}}.
\]
Moreover, we have 
\[
    \Delta_1(q) = \sqrt{\fr{\Phi'_1(q)}{(\xi^1 \circ \Phi)'(q)}}
\]
almost everywhere on $[q_1,1]$.
Analogous equations hold with $s$ in place of $1$.
\bhcomment{appeal to some regularity here, below not totally rigorous}

The definitions of $\Delta_s(q)$ imply that
\[
    \zeta(q) = -\fr{1}{\Phi'_s(q)} \fr{\de}{\de q} \sqrt{\fr{\Phi'_1(q)}{(\xi^1 \circ \Phi)'(q)}}
\]
for all $s\in \sS$, i.e. $\Phi$ solves the type II ode on $[q_1,1]$.
Moreover comparing the two formulas for $\Delta$ above we get
\[
    \fr{\Phi'_1(q_1)}{(\xi^1 \circ \Phi)'(q_1)} = \fr{\Phi_1(q_1)}{(\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1}
\]
and similarly for all $s\in \sS$, i.e. $\Phi(q_1)$ is solvable.
Construct $(p,\Phi,q_0)$ by making $p=1$ and $\Phi$ as above on $[q_1,1]$, and define $q_0$ and $(p,\Phi)$ on $[q_0,q_1]$ as the type I extension of $\Phi(q_1)$.
We can plug this into the alg functional, so $\ALG = \OPT$.

% Here $\psi$ is supported on $[q_1,1]$ with $\psi(1)=0$ (but not necessarily $\psi(q_1)=0$).
% Then 
% \[
%     \fr{\de}{\de \delta} (\xi^s \circ \Phi)(q) 
%     = 
%     (\psi \times \partial_1 \xi^s \circ \Phi)(q)
%     =
%     \fr{\lambda_s}{\lambda_1} (\psi \times \partial_s \xi^1 \circ \tPhi)(q),
%     \qquad
%     \fr{\de}{\de \delta} \Delta_1(q) 
%     = 
%     \int_q^1 \zeta(t) \psi'(t)~\de t
% \]
% and $\Delta_s(q)$ for $s\neq 1$ does not change under the perturbation.
% Now,
% \begin{align*}
%     F_1 
%     &\equiv
%     \fr{\de}{\de \delta}
%     2 \lambda_1^{-1} \CS_1 \Big|_{\delta=0} \\
%     &= 
%     \fr{\psi(q_1)}{\Delta_1(q_1)} 
%     + \sum_{s\in \sS} 
%     (\psi \times \partial_s \xi^1 \circ \Phi)(q_1) \Delta_s(q_1)
%     + \lt(
%         -\fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
%         +\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
%     \rt) \lt(
%         \int_{q_1}^1 \zeta(t) \psi'(t) ~\de t
%     \rt).
% \end{align*}
% Moreover,
% \[
%     F_2 
%     \equiv 
%     \fr{\de}{\de \delta}
%     2 \lambda_1^{-1} \CS_2 \Big|_{\delta=0} 
%     = F_{2,1} + F_{2,2} + F_{2,3} 
% \]
% for
% \begin{align*}
%     F_{2,1}
%     &= 
%     \int_{q_1}^1 \fr{\psi'(q)}{\Delta_1(q)} ~\de q 
%     = 
%     -\fr{\psi(q_1)}{\Delta_1(q_1)} 
%     -\int_{q_1}^1 
%     \fr{\psi(q) \zeta(q) \Phi'_1(q)}{\Delta_1(q)^2} ~\de q \\
%     F_{2,2}
%     &= 
%     \sum_{s\in \sS}
%     \int_{q_1}^1 
%     (\psi \times \partial_s\xi^1 \circ \Phi)'(q) 
%     \Delta_s(q) ~\de q \\
%     &=
%     - \sum_{s\in \sS}
%     (\psi \times \partial_s\xi^1 \circ \Phi)(q_1)\Delta_s(q_1) 
%     + \sum_{s\in \sS} 
%     \int_{q_1}^1 
%     \psi(q) \zeta(q) (\partial_s \xi^1 \circ \Phi)(q) \Phi'_s(q) 
%     ~\de q\\
%     &=
%     - \sum_{s\in \sS}
%     (\psi \times \partial_s\xi^1 \circ \Phi)(q_1)\Delta_s(q_1) 
%     +
%     \int_{q_1}^1 
%     \psi(q) \zeta(q) (\xi^1 \circ \Phi)'(q) 
%     ~\de q \\
%     F_{2,3}
%     &= 
%     \int_{q_1}^1 \lt(
%         -\fr{\Phi'_1(q)}{\Delta_1(q)^2}
%         + (\xi^1 \circ \Phi)'(q)
%     \rt)\lt(
%         \int_q^1 \zeta(t) \psi'(t) ~\de t
%     \rt) ~\de q.
% \end{align*}
% Thus
% \begin{align*}
%     &\fr{\de}{\de \delta}
%     \CS(\zeta,\tPhi,\vDelta) \Big|_{\delta = 0} \\
%     &= 
%     \lt(
%         -\fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
%         +\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
%     \rt) \lt(
%         \int_{q_1}^1 \zeta(t) \psi'(t) ~\de t
%     \rt) \\
%     &\quad +
%     \int_{q_1}^1 
%     \lt(
%         -\fr{\Phi'_1(q)}{\Delta_1(q)^2}
%         + (\xi^1 \circ \Phi)'(q)
%     \rt)\lt(
%         \psi(q) \zeta(q) +
%         \int_q^1 \zeta(t) \psi'(t) ~\de t
%     \rt) ~\de q \\
%     &= 
%     \lt(
%         \fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
%         -\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
%     \rt) \lt(
%         \psi(q_1) \zeta(q_1) 
%         + \int_{q_1}^1 \psi(t) \zeta'(t) ~\de t
%     \rt) \\
%     &\quad +
%     \int_{q_1}^1 
%     \lt(
%         \fr{\Phi'_1(q)}{\Delta_1(q)^2}
%         - (\xi^1 \circ \Phi)'(q)
%     \rt)\lt(
%         \int_q^1 \psi(t) \zeta'(t) ~\de t
%     \rt) ~\de q \\
%     &= 
%     \psi(q_1) \zeta(q_1) \lt(
%         \fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
%         -\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
%     \rt) \\
%     &\quad + 
%     \int_{q_1}^1 
%     \psi(q) \zeta'(q) \lt(
%         \fr{\Phi_1(q_1)}{\Delta_1(q_1)^2} 
%         -\lt((\xi^1 \circ \Phi)(q_1) + h_1^2/\lambda_1\rt)
%         + 
%         \int_{q_1}^q 
%         \lt(
%             \fr{\Phi'_1(t)}{\Delta_1(t)^2}
%             - (\xi^1 \circ \Phi)'(t)
%         \rt)
%         ~\de t
%     \rt) 
%     ~\de q.
% \end{align*}


==> final-tex/a3-asymmetric-maximizers.tex <==
\section{Asymmetric Maximizers for Symmetric $\xi$ }
\label{sec:non-unique}

Let 
\[
    \xi(x,y)=x^4+y^4+24xy.
\]
This function is symmetric in $(x,y)$. We will show that the natural minimizer is not symmetric via a 2nd derivative expansion.


We wish to compute $\deriv{\delta}G$. Here we fix $\chi\in C_c^{\infty}((0,1);\mathbb R)$ (hence $\chi(0)=\chi(1)=0$) and set
\[
    \Phi_1^{\delta\chi}(q)
    =
    \Phi^*_1(q) 
    +
    \delta
    \chi(q)
\]
so that
\[
    (\Phi_1^{\delta\chi})'(q)
    =
    (\Phi^*_1)'(q) + \delta \chi'(q)
\]
for all $q\in [0,1]$. As before let $\Phi_s^{\delta\chi}=\Phi_s^*$ for $s\neq 1$. Similarly to before we compute:
\begin{align*}
    \deriv{\delta} (\Phi_1^{\delta\chi})'(q)
    &=
    \chi'(q)
    ;
    \\
    \deriv{\delta} \Phi_1^{\delta\chi}(q)
    &=
    \chi(t)
    ;
    \\
    \deriv{\delta} (\xi^s \circ \Phi)'(q)
    &=
    \deriv{q} \lt((\partial_1\xi^s \circ \Phi)(q) \chi(q)\rt).
\end{align*} 
We will use the computation
\[
    \lt(\sqrt{\frac{f}{g}}\rt)' = \frac{f'g-fg'}{2f^{1/2}g^{3/2}}.
\] 
Recall the previous calculation and setting $p\equiv 1$, we find
\begin{align*}
    G(\Phi,\chi)&
    \equiv 2\deriv{\delta} F(\Phi^{\delta\chi}) \Big|_{\delta = 0} \\
    &=
    \lambda_1
    \underbrace{
        \int_0^1
        \sqrt{\frac{(\xi^1 \circ \Phi)'(q)}{\Phi'_1(q)}}
        \chi'(q)
        \diff{q}
    }_{T_0}
    +
    \sum_{s\in \sS}
    \lambda_s
    \underbrace{
        \int_0^1
        \sqrt{\fr{\Phi'_s(q)}{( \xi^s \circ \Phi)'(q)}}
        \deriv{\delta} ( \xi^s \circ \Phi^{\delta\chi})'(q)
        \Big|_{\delta=0}
        \diff{q}
    }_{T_s}.
\end{align*}



We now begin the main computation with:
\begin{align*}
    \deriv{\delta} T_0
    &=
    \int_0^1 
    \deriv{\delta}
    \lt(
        \sqrt{
        \frac
        {(\xi^1\circ\Phi^{\delta})'(q)}
        {(\Phi_1^{\delta})'(q)}
        }
    \rt)
    \chi'(q)
    \de q
    \\
    &=
    \frac{1}{2}
    \int_0^1 
    \frac{
        \deriv{q} \lt((\partial_1\xi^1 \circ \Phi)(q) \chi(q)\rt)\Phi_1'(q)
        -
        (\xi^1\circ\Phi^{\delta})'(q)\chi'(q)
    }
    {
    (\xi^1\circ\Phi^{\delta})'(q)^{1/2}
    ~
    \Phi_1'(q)^{3/2}
    }
    \chi'(q)
    \de q
\end{align*}
When $\Phi(q)=(q,q)$ this simplifies to:
\begin{align*}
\deriv{\delta} T_0
    &=
    \frac{1}{2}
    \int_0^1 
    \frac{
        \deriv{q} \lt((\partial_1\xi^1 \circ \Phi)(q) \chi(q)\rt)\Phi_1'(q)
        -
        (\xi^1\circ\Phi^{\delta})'(q)\chi'(q)
    }
    {
    (\xi^1\circ\Phi^{\delta})'(q)^{1/2}
    ~
    \Phi_1'(q)^{3/2}
    }
    \chi'(q)
    \de q
    \\
    &=
    \frac{1}{2}
    \int_0^1 
    \frac{
        \deriv{q} \lt((\partial_1\xi^1)(q,q) \chi(q)\rt)
        -
        (\xi^1)'(q,q)\chi'(q)
    }
    {
    (\xi^1)'(q,q)^{1/2}
    }
    \chi'(q)
    \de q
    \\
    &=
    \frac{1}{2}
    \int_0^1 
    \frac{
        (\partial_1\xi^1)'(q,q) \chi(q)
        +
        \big(
            \partial_1\xi^1(q,q)-(\xi^1)'(q,q)
        \big)
        \chi'(q)
    }
    {
    (\xi^1)'(q,q)^{1/2}
    }
    \chi'(q)
    \de q
    \\
    &=
    \frac{1}{2}
    \int_0^1 
    \frac{
        (\partial_1\xi^1)'(q,q) \chi(q)
        -
        \partial_2\xi^1(q,q)
        \chi'(q)
    }
    {
    (\xi^1)'(q,q)^{1/2}
    }
    \chi'(q)
    \de q
\end{align*}



Next we write things out for $T_s$:
\begin{align*}
    \deriv{\delta} T_s
    &=
    \int_0^1
    \deriv{\delta}
    \lt(
    \sqrt{
        \frac
        {(\Phi_s^{\delta})'(q)}
        {(\xi^s\circ\Phi^{\delta})'(q)}
    }
    \deriv{q} \lt((\partial_1\xi^s \circ \Phi^{\delta})(q) \chi(q)\rt)
    \rt)
    \de q
    \\
    &=
    \int_0^1
    \lt(
    \sqrt{
        \frac
        {(\Phi_s)'(q)}
        {(\xi^s\circ\Phi)'(q)}
    }
    \deriv{q} \lt((\partial_{1,1}\xi^s \circ \Phi)(q) \chi(q)^2\rt)
    \rt)
    \de q
    \\
    &\quad\quad\quad
    +
    \int_0^1
    \deriv{\delta}
    \lt(
    \sqrt{
        \frac
        {(\Phi_s^{\delta})'(q)}
        {(\xi^s\circ\Phi^{\delta})'(q)}
    }
    \rt)
    \deriv{q} \big((\partial_1\xi^s \circ \Phi)(q) \chi(q)\big)
    \de q
    .
\end{align*}
With $\Phi(q)=(q,q)$ we have the intermediate computations
\begin{align*}
    \deriv{q} \lt((\partial_{1,1}\xi^1 \circ \Phi)(q) \chi(q)^2\rt)
    &=
    (\partial_{1,1}\xi^s\circ\Phi)'(q)\chi(q)^2
    +
    2(\partial_{1,1}\xi^s\circ\Phi)(q)\chi(q)\chi'(q)
    \\
    &=
    \partial_{1,1}\xi^s(q,q)'\chi(q)^2 + \big(2\partial_{1,1}\xi^s(q,q)\big)\chi(q)\chi'(q)
    .
\end{align*}
For the other term, in the case $s=1$ we have
\begin{align*}
    \deriv{\delta}
    \lt(
    \sqrt{
        \frac
        {(\Phi_1^{\delta})'(q)}
        {(\xi^1\circ\Phi^{\delta})'(q)}
    }
    \rt)
    &=
    \frac{
        \deriv{\delta}(\Phi_1^{\delta})'(q)
        \times
        (\xi^1\circ\Phi^{\delta})'(q)
        -
        (\Phi_1^{\delta})'(q)
        \deriv{\delta}
        (\xi^1\circ\Phi^{\delta})'(q)
    }
    {2(\Phi_1^{\delta})'(q)^{1/2}~(\xi^1\circ\Phi^{\delta})'(q)^{3/2}}
    \\
    &=
    \frac{
        \chi'(q)
        (\xi^1\circ\Phi)'(q)
        -
        (\Phi_1)'(q)
        \deriv{q} \lt((\partial_1\xi^1 \circ \Phi)(q) \chi(q)\rt)
    }
    {2(\Phi_1)'(q)^{1/2}~(\xi^1\circ\Phi)'(q)^{3/2}}
     \\
    &=
    \frac{
        \chi'(q)
        \xi^1(q,q)'
        -
        \deriv{q} \lt((\partial_1\xi^1(q,q) \chi(q)\rt)
    }
    {2(\xi^1(q,q)')^{3/2}}
     \\
    &=
    \frac{
        \chi'(q)
        \partial_2\xi^1(q,q)
        -
        \chi(q)\partial_1\xi^1(q,q)' 
    }
    {2(\xi^1(q,q)')^{3/2}}
\end{align*}
while for $s=2$
\begin{align*}
    \deriv{\delta}
    \lt(
    \sqrt{
        \frac
        {(\Phi_2^{\delta})'(q)}
        {(\xi^2\circ\Phi^{\delta})'(q)}
    }
    \rt)
    &=
    \frac{
        \deriv{\delta}(\Phi_2^{\delta})'(q)
        \times
        (\xi^2\circ\Phi^{\delta})'(q)
        -
        (\Phi_2^{\delta})'(q)
        \deriv{\delta}
        (\xi^2\circ\Phi^{\delta})'(q)
    }
    {2(\Phi_2^{\delta})'(q)^{1/2}~(\xi^2\circ\Phi^{\delta})'(q)^{3/2}}
    \\
    &=
    \frac{
        -
        \Phi_2'(q)
        \deriv{q} \lt((\partial_1\xi^2 \circ \Phi)(q) \chi(q)\rt)
    }
    {2\Phi_2'(q)^{1/2}~(\xi^2\circ\Phi)'(q)^{3/2}}
     \\
    &=
    \frac{
        -
        \deriv{q} \lt((\partial_1\xi^2(q,q) \chi(q)\rt)
    }
    {2(\xi^2(q,q)')^{3/2}}
     \\
    &=
    \frac{
        -
        \partial_1\xi^2(q,q)' \chi(q)
        -
        \partial_1\xi^2(q,q)\chi'(q)
    }
    {2(\xi^2(q,q)')^{3/2}}.
\end{align*}
Additionally,
\begin{align*}
    \deriv{q} \lt((\partial_1\xi^s \circ \Phi)(q) \chi(q)\rt)
    &=
    \partial_1\xi^s(q,q)'\chi(q) + \partial_1\xi^s(q,q)\chi'(q).
\end{align*}

We found above that
\begin{align*}
    \deriv{\delta} T_s
    &=
    \int_0^1
    \lt(
    \sqrt{
        \frac
        {(\Phi_s)'(q)}
        {(\xi^s\circ\Phi)'(q)}
    }
    \deriv{q} \lt((\partial_{1,1}\xi^s \circ \Phi)(q) \chi(q)^2\rt)
    \rt)
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \deriv{\delta}
    \lt(
    \sqrt{
        \frac
        {(\Phi_s^{\delta})'(q)}
        {(\xi^s\circ\Phi^{\delta})'(q)}
    }
    \rt)
    \deriv{q} \lt((\partial_1\xi^s \circ \Phi)(q) \chi(q)\rt)
    \de q
    .
\end{align*}
In particular $s=1$ gives
\begin{align*}
    \deriv{\delta} T_1
    &=
    \int_0^1
    \frac
    {1}
    {(\xi^1(q,q)')^{1/2}}
    \lt(
        (\partial_{1,1}\xi^1(q,q))'\chi(q)^2 + 2\big(\partial_{1,1}\xi^1(q,q)\big)\chi(q)\chi'(q)
    \rt)
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac{
        \chi'(q)
        \partial_2\xi^1(q,q)
        -
        \chi(q)\partial_1\xi^1(q,q)' 
    }
    {2(\xi^1(q,q)')^{3/2}}
    \lt(
        \partial_1\xi^1(q,q)'\chi(q) + \partial_1\xi^1(q,q)\chi'(q)
    \rt)
    \de q
\end{align*}
and $s=2$ gives
\begin{align*}
    \deriv{\delta} T_2
    &=
    \int_0^1
    \frac
    {1}
    {(\xi^2(q,q)')^{1/2}}
    \lt(
        (\partial_{1,1}\xi^2(q,q))'\chi(q)^2 + 2\big(\partial_{1,1}\xi^2(q,q)\big)\chi(q)\chi'(q)
    \rt)
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac{
        -
        \partial_1\xi^2(q,q)' \chi(q)
        -
        \partial_1\xi^2(q,q)\chi'(q)
    }
    {2(\xi^2(q,q)')^{3/2}}
    \lt(
        \partial_1\xi^2(q,q)'\chi(q) + \partial_1\xi^2(q,q)\chi'(q)
    \rt)
    \de q.
\end{align*}
Moreover since $\xi(x,y)=x^4+y^4+24xy$, we have
\begin{align*}
    \partial_2\xi^1(q,q)
    =
    \partial_1\xi^2(q,q)
    =
    \frac{24}{\lambda_s}
    &=
    48
    \\
    \partial_{1}\xi^2(q,q)'&=0
    \\
    \partial_{1,1}\xi^2(q,q)&=0.
\end{align*}
Additionally,
\begin{align*}
    (\partial_1\xi^1)'(q,q)&=
    \partial_{1,1}\xi^1(q,q)
    \\
    &=
    2\partial_{x,x,x}\xi(x,y)|_{x=y=q} 
    \\
    &= 48q;
    \\
    (\partial_{1,1}\xi^1(q,q))'&=48;
    \\
    \xi^1(q,q)'=\xi^2(q,q)'&=24q^2+48;
    \\
    \partial_1\xi^1(q,q)&=24q^2
    .
\end{align*}


We combine our computations below. The red line vanishes since $\partial_{1,1}\xi^2(x,y)\equiv 0$.
\begin{align*}
    2\deriv{\delta}G
    &=
    \deriv{\delta}(T_0+T_1+T_2)
    \\
    &=
    \frac{1}{2}
    \int_0^1 
    \frac{
    (\partial_1\xi^1)'(q,q) \chi(q)
    -
    \partial_2\xi^1(q,q)
    \chi'(q)
    }
    {
    (\xi^1)'(q,q)^{1/2}
    }
    \chi'(q)
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac
    {1}
    {(\xi^1(q,q)')^{1/2}}
    \lt(
        (\partial_{1,1}\xi^1(q,q))'\chi(q)^2 + 2\big(\partial_{1,1}\xi^1(q,q)\big)\chi(q)\chi'(q)
    \rt)
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac{
        \chi'(q)
        \partial_2\xi^1(q,q)
        -
        \chi(q)\partial_1\xi^1(q,q)' 
    }
    {2(\xi^1(q,q)')^{3/2}}
    \lt(
        \partial_1\xi^1(q,q)'\chi(q) + \partial_1\xi^1(q,q)\chi'(q)
    \rt)
    \de q
    \\
    &\quad\quad\quad+
    {
        \color{red}
        \int_0^1
        \frac
        {1}
        {(\xi^2(q,q)')^{1/2}}
        \lt(
            (\partial_{1,1}\xi^2(q,q))'\chi(q)^2 + 2\big(\partial_{1,1}\xi^2(q,q)\big)\chi(q)\chi'(q)
        \rt)
        \de q 
    }
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac{
        -
        \partial_1\xi^2(q,q)' \chi(q)
        -
        \partial_1\xi^2(q,q)\chi'(q)
    }
    {2(\xi^2(q,q)')^{3/2}}
    \lt(
        \partial_1\xi^2(q,q)'\chi(q) + \partial_1\xi^2(q,q)\chi'(q)
    \rt)
    \de q.
    \\
    %%%%%%%%
    &=
    %%%%%%%%
    \frac{1}{2}
    \int_0^1 
    \frac{
    48q\chi(q)
    -
    48
    \chi'(q)
    }
    {
    (24q^2+48)^{1/2}
    }
    \chi'(q)
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac
    {
    \lt(
        48\chi(q)^2 + 96q\chi(q)\chi'(q)
    \rt)
    }
    {(24q^2+48)^{1/2}}
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac{
        48\chi'(q)
        -
        48q\chi(q)
    }
    {2(24q^2+48)^{3/2}}
    \lt(
        48q\chi(q) + 24q^2\chi'(q)
    \rt)
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac{
    -48\chi'(q)
    }
    {2(24q^2+48)^{3/2}}
    \lt(
        48\chi'(q)
    \rt)
    \de q    
    \\
    %%%%%%%%v2
    &=
    %%%%%%%%v2
    \sqrt{24}
    \int_0^1 
    \frac{
    q\chi(q)
    -
    \chi'(q)
    }
    {
    (q^2+2)^{1/2}
    }
    \chi'(q)
    \de q
    \\
    &\quad\quad\quad+
    \sqrt{24}
    \int_0^1
    \frac
    {
    \lt(
        2\chi(q)^2 + 4q\chi(q)\chi'(q)
    \rt)
    }
    {(q^2+2)^{1/2}}
    \de q
    \\
    &\quad\quad\quad+
    \sqrt{24}
    \int_0^1
    \frac{1}
    {(q^2+2)^{3/2}}
    \Big(
    \big(
        \chi'(q)-q\chi(q)
    \big)
    \cdot
    \big(
        2q\chi(q) + q^2\chi'(q)
    \big)
    -
    2\chi'(q)^2
    \Big)
    \de q.
\end{align*}


Simplifying further,
\begin{align*}
    \frac{\deriv{\delta}G}{\sqrt 6}
    &=
    \int_0^1 
    \frac{
    q\chi(q)
    -
    \chi'(q)
    }
    {
    (q^2+2)^{1/2}
    }
    \chi'(q)
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac
    {
    \lt(
        2\chi(q)^2 + 4q\chi(q)\chi'(q)
    \rt)
    }
    {(q^2+2)^{1/2}}
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac{1}
    {(q^2+2)^{3/2}}
    \Big(
    \big(
        \chi'(q)-q\chi(q)
    \big)
    \cdot
    \big(
        2q\chi(q) + q^2\chi'(q)
    \big)
    -
    2\chi'(q)^2
    \Big)
    \\
    %%%
    &=
    %%%
    \int_0^1 
    \frac{
    1
    }
    {
    (q^2+2)^{1/2}
    }
    \lt(
    2\chi(q)^2 + 5q\chi(q)\chi'(q)-\chi'(q)^2
    \rt)
    \de q
    \\
    &\quad\quad\quad+
    \int_0^1
    \frac{1}
    {(q^2+2)^{3/2}}
    \Big(
    \big(
        \chi'(q)-q\chi(q)
    \big)
    \cdot
    \big(
        2q\chi(q) + q^2\chi'(q)
    \big)
    -
    2\chi'(q)^2
    \Big)
    \de q
    .
\end{align*}
Note that this is a quadratic form in $(\chi(q),\chi'(q))$ as we expect. Now we want to find an example function $\chi$ making this strictly positive. This will show that $\Phi(q)=(q,q)$ is \textbf{not} a local maximum for the ALG functional. 

We try
\begin{align*}
    \chi(q)&=\sin(\pi cq);
    \\
    \chi'(q)&=\pi c\cos(\pi cq).
\end{align*}
on $q\in [0,1/c]$, for $c=\frac{1}{10}$ and $c=\frac{1}{20}$. 

\begin{figure}[h]
\includegraphics[width=0.45\linewidth]{imgs/wolfram-pic-10.png}
\includegraphics[width=0.45\linewidth]{imgs/wolfram-pic-20.png}
\caption{This calculation showcases the beauty of the multi-species setting.}
\end{figure}


It would be good to numerically verify the above calculations by manually computing ALG. Once that seems ok, it would be nice to look into a rigorous numerical integrator. (Although the integrand seems tame enough to trust Wolfram Alpha.)


==> final-tex/a4-state-evolution.tex <==
\section{State Evolution: Proof of Proposition \ref{prop:state_evolution}}
\label{sec:ProofSE}


In this section we prove Proposition~\ref{prop:state_evolution}, following the appendix of \cite{ams20}. Throughout, we denote by $\bG^{(k)}\in (\bbR^N)^{\otimes k}$, $k\ge 2$ a sequence of standard Gaussian tensors. For $S_k$ the symmetric group on $k$ elements we also write 
\begin{equation}
\label{eq:Ak-def}
    \bA^{(k)}=\frac{1}{N^{(k-1)/2} }\Gamma^{(k)}
    \diamond 
    \sum_{\pi\in S^k}(\bG^{(k)})^{\pi}
\end{equation}
for the rescaled tensors with entries
\begin{equation}
\label{eq:A-defn}
     \bA^{(k)}_{i_1,\dots,i_k}
     =
     \frac{1}{N^{(k-1)/2} }
     \gamma_{s(i_1),\dots,s(i_k)} 
     \sum_{\pi\in S_k}\bG^{(k)}_{i_{\pi(1)},\dots,i_{\pi(k)}}
     \,.
\end{equation}
For a symmetric tensor $\bA^{(k)}\in(\bbR^N)^{\otimes k}$ and $\bT\in(\bbR^N)^{\otimes (k-1)}$, we denote by  $\bA^{(k)}\{\bT\}\in\bbR^N$ the vector with components
\begin{equation}
\label{eq:TensorTensor}
    \bA^{(k)}\{\bT\}_i = \frac{1}{(k-1)!}\sum_{1\le i_1,\cdots,i_{k-1}\le N}A^{(k)}_{i,i_1,\cdots,i_{k-1}}T_{i_1\dots i_{k-1}}.
\end{equation}
For $\bu\in\bbR^N$ we denote by $\bA^{(k)}\{\bu\}=\bA^{(k)}\{\bu^{\otimes (k-1)}\}$ the vector with entries
%
\begin{equation}
\label{eq:vector}
\bA^{(k)}\{\bu\}_i = \frac{1}{(k-1)!}\sum_{1\le i_1,\cdots,i_{k-1}\le N}A^{(k)}_{i,i_1,\cdots,i_{k-1}}u_{i_1}\cdots u_{i_{k-1}}.
\end{equation}
Note that for $\bA^{(k)}$ as in \eqref{eq:Ak-def}, one has 
\[
\bA^{(k)}\{\bu\}=\nabla H_{N,k}(\bu)
\]
where $H_{N,k}$ denotes the part of $H_N$ of total degree $k$.


For $\bu,\bv\in\bbR^N$ we recall from Subsection~\ref{subsec:notation} the notations 
\begin{align*}
    \< \bv\>_N&=N^{-1}\sum_{i\le N} v_i,
    \\
    \< \bu,\bv\>_N
    &= 
    N^{-1}\sum_{i\le N}u_iv_i
    =
    \langle\vec\lambda, \vR(\bu,\bv)\rangle,
    \\
    \|\bu\|_{N}&= \<\bu,\bu\>_N^{1/2}=\sqrt{\sum_s \lambda_s R_s(\bu,\bu)}.
\end{align*}


Given functions $f_{t,s}:\bbR^{t+1}\to\bbR$ of $t+1$
variables for each $s\in\sS$, and $\bv^0,\bv^1,\dots,\bv^t\in\bbR^{N}$, we define $f_t(\bv^0,\bv^1,\dots,\bv^t)\in\mathbb R^N$ component-wise via
%
\begin{align}
%
    f_t(\bv^0,\bv^1,\dots,\bv^t)_i=f_{t,s(i)}(v^0_i,\dots,v^t_i).
%
\end{align}
%
Finally, for a sequence of vectors $\bw^0,\bw^1,\dots$, we write $\bw^{\le t} = (\bw^0,\bw^1,\dots,\bw^t)$.


To deduce the state evolution result for mixed tensors, we analyze a slightly more general iteration where each homogenous
$k$-tensor is tracked separately, while restricting ourselves to the case where the mixture $\xi$ has finitely many components: $\gamma_{s_1,\dots,s_k} = 0$ for all $(s_1,\dots,s_k)\in \sS^k$ for all $k \ge D +1$ for some fixed $D \ge 2$. We then proceed by an approximation argument to extend the convergence to the general case $D = \infty$.

We begin by introducing the Gaussian process that captures the asymptotic behavior of AMP. 
Define $\xi^k$ to be the degree $k$ part of $\xi$, and 
\[
    \xi^{k,s}=\frac{1}{\lambda_s}\partial_{x_s}\xi^k(x_1,\dots,x_r)
\]
the degree $k-1$ part of $\xi^s$. 

An AMP iteration is specified by Lipschitz functions $f_{t,s}:\bbR^{2(t+1)}\to \bbR$ for each $(t,s)\in\naturals\times \sS$.\footnote{The unusual factor $2$ in the exponent comes from the external randomness vectors $\be^1,\dots,\be^t$.}  
For each iteration $t$, the state of the algorithm is given by vectors
$\bw^t\in \bbR^N$, and $\bz^{k,t}\in \bbR^N$, with $k\in\{2,\dots,D\}$. 
Moreover for each $t$, there is also an external randomness vector $\be^t\in\bbR^N$ with independent coordinates $e^t_i\sim \mu_{t,s(i)}$ from deterministic probability distributions $\big(\mu_{t,s}\big)_{t\geq 0,s\in \sS}$ with finite $L^2$ norm.
We now start to define the AMP iteration steps (the definition finishes at \eqref{eq:recursive-covariance}). A single step is given by
%
\begin{align}
\label{eq:AMP-def1}
    \AMP_t
    \lt(\bw^0,\dots,\bw^t
    ;
    \be^0,\dots,\be^t\rt
    )_{k}
    &\equiv
    \bA^{(k)}
    \{
    \f_t
    \}
    -
    \sum_{t'\leq t}
    d_{t,t',k}
    \diamond 
    \f_{t'-1}
    \, ,
    \\
\label{eq:bff}
    \f_t &= f_t(\bw^0,\dots,\bw^t;\be^0,\dots,\be^t),
    \\
\label{eq:AMP-def2}
    d_{t,t',k,s} 
    &\equiv 
    \sum_{s'\in\sS}
    \partial_{x_{s'}}\xi^{k,s}
    \lt(\lt( 
    \E\lt[ 
    F_{t,s} F_{t'-1,s}
    \rt]
    \rt)_{s\in\sS}
    \rt) 
    \times
    \E\lt[ 
    \frac{\partial_{W^{t'}_{s'}} F_{t,s'}}{\partial W^{t'}_{s'}}
    \rt]
    \, 
    ,
    \\
\label{eq:F-def}
    F_{t,s'}
    &\equiv
    f_{t,s'}\big(W^0_{s'},W^1_{s'},\dots, W^t_{s'};E^0_{s'},\dots,E^t_{s'}\big)
    .
%
\end{align}
A general multi-species tensor AMP algorithm then takes the form:
\begin{align}
\label{eq:TensorAMP}
    \bw^t=\sum_{2\leq k\leq D} \bz^{k,t}\, ,\quad \quad
    \bz^{k,t+1}
    =
    \AMP_t
    \lt(\bw^0,\dots,\bw^t;\be^0,\dots,\be^t\rt)_k\, .
\end{align}


For the right-hand side of \eqref{eq:F-def} to make sense, we must define for each $t\geq 0$ and $s\in \sS$ a distribution over sequences
$(W^0_s,\dots,W^t_s;E^0_s,\dots,E^t_s)$. The latter variables $E^{t'}_s\sim \mu_{t',s}$ are simply taken independent of each other and all other variables. The construction of the $W$ variables is recursive across $t$ as follows. 
For each $2\leq k\leq D$ and $s\in\sS$, we let $U^{k,0}_s\sim \nu_{k,s}$
and construct a centered Gaussian process
\[
    (U^{k,1}_s,U^{k,1}_s,\dots,U^{k,t}_s)
\]
which is independent of $U^{k,0}_s$. The variables $U^{k,t}_s$ and $U^{k',t'}_{s'}$ are independent unless $(k,s)=(k',s')$. It remains to specify the covariance of $(U^{k,t}_s)_{1\leq t\le T}$ which is given recursively by:
\begin{equation}
\label{eq:recursive-covariance}
\begin{aligned}
    \E\big[U^{k,t+1}_s U^{k,t'+1}_{s}\big]
    & = 
    \xi^{k,s}(\Sigma^{k,t,t'})\,;
    \\
    \Sigma^{k,t,t'}_{s}
    &=
    \bbE\lt[
    f_{t,s}(W^0_s,\dots,W^t_s;E^0_s,\dots,E^t_s)
    f_{t',s}(W^0_s,\dots,W^{t'}_s;E^0_s,\dots,E^{t'}_s)
    \rt],\quad \forall s\in \sS
    \\
    W^t_s & \equiv  \sum_{2\leq k\leq D} U^{k,t}_s\, 
    .
\end{aligned}
\end{equation}





%
The main result, an extension of Proposition \ref{prop:state_evolution}, follows. Below we use $\bbW_2$ to denote the Wasserstein-$2$ distance between probability measures on Euclidean space in any dimension. We say a function $\psi:\bbR^d\to\bbR$ is \textbf{pseudo-Lipschitz} if 
\[
    |\psi(\bw)-\psi(\by)|
    \leq 
    C(1+\|\bw\|+\|\by\|)
    \cdot 
    \|\bw-\by\|
    ,\quad\forall \bw,\by\in\bbR^d.
\]

\begin{theorem}[State Evolution for AMP]
\label{thm:mixedAMP}
Let $\{\bG^{(k)}\}_{k\ge 2}$ be independent standard Gaussian tensors with $\bG^{(k)}\in(\bbR^N)^{\otimes k}$, and define $\bA^{(k)}$ as in \eqref{eq:A-defn}. Fix a sequence of Lipschitz functions $f_{t,s}:\bbR^{k+1}\to\bbR$.
 Let $\bz^{2,0},\cdots \bz^{D,0}\in\bbR^N$ be deterministic vectors and $\bw^0 =\sum_{2\leq k\leq D} \bz^{k,0}$.
Assume that for each $s\in\sS$, the empirical distribution of the vectors 
\[
    (z_i^{2,0},\cdots z_i^{D,0}),\quad i\in \cI_s
\]
converges in $\bbW_2(\bbR^{D-1})$ distance to the law of the vector $(U^{k,0}_s)_{2\le k\le D}$. 

Let $\bw^{t}, \bz^{k,t}$, $t\ge 1$ be given by the \emph{tensor AMP} iteration. Then, for all $s\in\sS$ and $T\ge 1$ and for any pseudo-Lipschitz functions $\psi:\bbR^{D \times T}\to \bbR$ and $\wt\psi:\bbR^T\to\bbR$, we have
%
\begin{align}
\label{eq:z-U-convergence}
    \plim_{N\to\infty}\frac{1}{N_s}\sum_{i\in\cI_s}\psi \Big((z_i^{k,t})_{ k\le D,t\le T}\Big) 
    &= \E\lt[\psi\big((U^{k,t}_s)_{2\leq k\leq D,t\leq T}\big)\rt]\, 
    ;
    \\
\label{eq:w-W-convergence}
    \plim_{N\to\infty}\frac{1}{N_s}\sum_{i\in\cI_s}\wt\psi \Big((w_i^{t})_{t\le T}\Big) 
    &= \E\lt[\wt\psi\big((W^{t}_s)_{t\leq T}\big)\rt]\,
    .
%
\end{align}
\end{theorem}
%

Note that \eqref{eq:w-W-convergence} (which concerns the actual AMP iterates $\bw^t$) is a special case of \eqref{eq:z-U-convergence} (which is more convenient to prove). Indeed one can take $\psi((z^{k,t})_{k\le D,t\le T}=\wt\psi\lt(\sum_{k\le D}z^{k,t}\rt)_{t\le T}$. 
In the special case that $c_k =0$ for all $k\ge D+1$, Proposition \ref{prop:state_evolution} follows immediately from Theorem~\ref{thm:mixedAMP} by baking the contribution of $\bh$ explicitly into $f_t$ (since we require $k\geq 2$ above). Proposition \ref{prop:state_evolution} for non-polynomial $\xi$ follows by a standard approximation argument outlined at the end of Subsection~\ref{subsec:further-def-app}.
For the remainder of this Appendix we thus focus on establishing \eqref{eq:z-U-convergence}.

\subsection{Further Definitions}
\label{subsec:further-def-app}

We define the notations
%
\begin{align*}
%
    \bW_t
    &=
    \big[
    \,\bw^0~|~\bw^1~|\;\cdots\;|~\bw^t
    \big]\, ,
    \\
    \bE_t
    &=
    \big[
    \,\be^0~|~\be^1~|\;\cdots\;|~\be^t
    \big]\, ,
    \\
    \bZ_{k,t}
    &=
    \big[
    \,\bz^{k,0}~|~\bz^{k,1}~|\,\cdots\;|~\bz^{k,t}\,
    \big].
\end{align*}
%
Given a $N\times (t+1)$ matrix such as $\bW_t$, and a tensor $\bA^{(k)}\in(\bbR^{N})^{\otimes k}$, we write 
$\bA^{(k)}\{\bW_t\}$ for the $N\times (t+1)$ matrix with columns $\bA^{(k)}\{\bw^0\}$, \dots, $\bA^{(k)}\{\bw^t\}$:
%
\begin{align*}
%
\bA^{(k)}\{\bW_t\}&=\Big[\bA^{(k)}\{\bw^0\}\Big|\bA^{(k)}\{\bw^1\}\Big|\;\cdots\;\Big|\bA^{(k)}\{\bw^t\}\Big]\, .
%
\end{align*}
%
We will write $\f_t=f_t(\W_t,\bE_t)=f_t(\bw^0,\dots,\bw^t,\be^0,\dots,\be^t)$ and also set 
%
\begin{align}
\label{eq:Ydef1}
    \by_{k,t+1}(\ZZ_{k,t})
    &=
    \A_k\lt\{\f_t\rt\} 
    = 
    \bz^{k,t+1}
    +
    \sum_{t_1\leq t} 
    d_{t,t_1,k}
    \diamond 
    \f_{t_1-1}\, ,
    \\
\label{eq:Ydef2}
    \bY_{k,t} 
    &= 
    [\by_{k,1}|\;\cdots\;|\by_{k,t}]
    \, ,
    \\
\nonumber
    \by_{t}(\ZZ_{k,t})&=\sum_{2\leq k\leq D}  \by_{k,t}(\ZZ_{k,t})\, . 
\end{align}
We also define an associated $(t+1)\times (t+1)$ Gram matrix $\bG_{\xi^{k,s}}=\bG_{\xi^{k,s},t}$ via 
\begin{equation}
\label{eq:bG-def}
    (\bG_{\xi^{k,s}})_{t_1,t_2}
    =
    \xi^{k,s}\big(\vR( 
    \f_{t_1},\f_{t_2})\big).
\end{equation}
The dependence of $\bG_{\xi^{k,s}}$ will often be suppressed.
We define a second Gram matrix 
$\bGG_{\xi^{k,s}}$, also of size $(t+1)\times (t+1)$, via (recall \eqref{eq:zeta-defn})
\begin{align}
\label{eq:bGG-def}
    (\bGG_{\xi^{k,s}})_{t_1,t_2}
    &=
    \zeta^{k,s}\lt(\vR\big( \f_{t_1},\f_{t_2}\big)\rt)
    \\
\nonumber
    &=
    \sum_{s'\in\sS}
    \partial_{x_{s'}}\xi^{k,s}
    \lt(\vR\big( \f_{t_1}, \f_{t_2}\big)\rt).
\end{align}
Finally, we let $\cF_t$ denote the $\sigma$-algebra generated by all iterates up to time $t$:
%
\begin{equation}
\label{eq:cFt-defn}
%
    \cF_t
    =
    \sigma\big(\{\bz_{k,t_1}\}_{k\le D,t_1\le t}\big)
    =
    \sigma\big(\{\bz_{k,t_1},\bw^{t_1},\f_{t_1}\}_{k\le D,t_1\le t}\big)\, .
%
\end{equation}

Throughout the proof of state evolution we make the following simplifying assumptions:

\begin{assumption}
\label{as:degree-D}
    $\xi$ is a degree $D$ polynomial with all coefficients $\gamma_{s_1,\dots,s_k}$ for $2\leq k\leq D$ strictly positive.
\end{assumption}

\begin{assumption}
\label{as:well-conditioned}
    Each matrix $\bG_{\xi^{k,s},t}$ is well-conditioned, i.e. 
    \[
    C^{-1}\le \sigma_{\min}(\bG_{\xi^{k,s},t})\le \sigma_{\max}(\bG_{\xi^{k,s},t})\le C
    \]
    for all $t\le T$. Here $\bG_{\xi^{k,s},t}$ is defined based on iterates that will appear in Theorems~\ref{thm:SELAMP} and \ref{lem:ampequalslamp}. The same holds for $\cL_{k,t}$ as defined in \eqref{eq:cL-k-t}.
\end{assumption}



It is a standard argument that to establish Proposition~\ref{prop:state_evolution}, it suffices to do so under the above assumptions. The reason is that one can always slightly perturb both $\xi$ and the non-linearities $f_{t,s}$ to ensure the assumptions hold. Then suitable continuity properties suffice to transfer all asymptotic guarantees. We refer the reader to \cite[Appendices A.8 and A.9]{ams20} for the arguments in the single-species case, still in the generality of mixed tensors. (In the more common setting $D=2$ of just a random matrix this step is also common for state evolution proofs, see e.g. \cite[Section 4.2.1]{javanmard2013state}.) The corresponding extension in our setting is completely analogous and omitted.




\subsection{Preliminary Lemmas}


The next lemma has several parts. All are elementary Gaussian calculations so their proofs are omitted.

\begin{lemma}
\label{lem:4}
For any deterministic $\bu,\bv\in \bbR^N$ and $\bA^{(k)}$ defined by \eqref{eq:A-defn} we have:
%
\begin{enumerate}
    \item Letting $g_0\sim\normal(0,1)$ be independent of $\bg\sim\normal(0,\id_N)$, we have
        \begin{align}
            \bA^{(k)}\{\bu\}\ed
            \sum_{s\in\sS}
            \bg_s
            \sqrt{\xi^{k,s}(\vR(\bu,\bu))}
            +  
            \frac{g_0}{\sqrt N}
            \sum_{s\in\sS}
            \bu_s
            \sqrt{
                \sum_{s'\in\sS}
                \partial_{x_{s'}} \xi^{k,s}
                \Big(
                \vR(\bu,\bu)
                \Big)
            }
            \, .
        \end{align}
    %
    \item Let $g_0,g_1,\dots,g_r\sim\normal(0,1)$ be independent. We have (jointly across $s\in\sS$)
    \begin{align}
        \sqrt{\lambda_s N} R_s(\bv,\bA^{(k)}\{\bu\})
        \ed 
        \sqrt{\xi^{k,s}(\vR(\bu,\bu))\cdot \vR(\bv,\bv)}g_s
        +  
        \sqrt{
            \sum_{s'\in\sS}
            \partial_{x_{s'}} \xi^{k,s}
            \Big(
            \vR(\bu,\bu)
            \Big)
        }
        R_s(\bu,\bv) \, g_0\, .
    \end{align}
    %
    \item For $s\in\sS$:
     \[
        R\lt(\bA^{(k)}\{\bu\},\bA^{(k)}\{\bv\}\rt)_s\simeq \xi^{k,s}\lt(\vR( \bu,\bv)\rt).
    \]
    \item For a deterministic symmetric tensor $\bT\in(\bbR^N)^{\otimes k-1}$, the vector
    $\bA^{(k)}\{\bT\}$ is centered Gaussian. Its covariance is given by
    %
    \begin{align*}
      \E\big[\bA^{(k)}\{\bT\}_i\bA^{(k)}\{\bT\}_j\big] 
      &= 
      \langle \xi^{k,s(i)}\diamond \bT,\, \bT\rangle_N
      \cdot 1\{i=j\} 
      \\
      &
      \quad
      +\frac{k(k-1)}{N^{k-1}}\,
      \sum_{i_1,\dots,i_{k-2}=1}^N
      \gamma_{i,i_1,\dots,i_{k-2}}
      \gamma_{j,i_1,\dots,i_{k-2}}
      T_{i,i_1,\dots,i_{k-2}}
      T_{j,i_1,\dots,i_{k-2}}\, . 
    \end{align*}
%
    \item Let $\bP\in\bbR^{N\times N}$ be the orthogonal projection onto a (deterministic) subspace $S\subseteq\bbR^N$ with $d=\dim(S)=O(1)$. Then
    \[
        \|\bP\bG^{(k)}\{\bu\} - \bG^{(k)}\{\bu\}\|_2 /\|\bG^{(k)}\{\bu\}\|_2\simeq 0.
    \]
\end{enumerate}
\end{lemma}
%



We next develop a formula for the conditional expectation of a Gaussian tensor $\bA^{(k)}$ given
a collection of linear observations.
We set $\bD$ to be the $t\times t\times t$ tensor with entries $D_{ijk}=1$ if $i=j=k$ and $D_{ijk}=0$ otherwise.
%
\begin{lemma}
\label{lem:symregression}
Recalling \eqref{eq:cFt-defn}, let $\E\{\bA^{(k)}|\cF_t\}$.
Equivalently $\E\{\bA^{(k)}|\cF_t\}$ is the conditional expectation of $\bA^{(k)}$ given the linear-in-$\bA^{(k)}$ observations
%
\begin{align}
%
\bA^{(k)}\{\f_{t'}\}=\by_{k,t'+1} \, \;\;\; \mbox{ for $s\in\{0,\dots,t-1\}$.} \label{eq:LinearConstraint}
%
\end{align}
%
Then we have for $i_1,i_2,\dots,i_k\leq n$,  
%
\begin{align}
%
\label{eq:SymmRegression}
    \E[\bA^{(k)}|\cF_t]_{i_1,i_2,\dots,i_k}= 
    \sum_{j=1}^k \sum_{0\leq r,s\leq t-1} (\hZZ_{k,t})_{i_j,s}\cdot (\bG^{-1}_{\xi^{k,s},t-1})_{s,r}\cdot (\f_{r,i_1}\cdots \f_{r,i_{j-1}}\f_{r,i_{j+1}}\cdots \f_{r,i_{k}})\, .
%
\end{align}
%
Here, the matrix $\hZZ_{k,t}\in\bbR^{N\times t}$ is defined as the solution of a system of linear equations as follows.
Define the linear operator $\cT_{k,t}:\bbR^{N\times t}\to\bbR^{N\times t}$ by letting, for $i\leq N$, $0\leq t_3\leq t-1$:
%
\begin{align}
\label{eq:Tdef}
    [\cT_{k,t}(\bZ)]_{i,t_3}&= \sum_{j=1}^N \sum_{0\leq t_1,t_2\leq t-1} (\f_{t_2})_{i} (\f_{t_2})_{j}
    \lt(
    (\bG_{\xi^{k,s(i)},t-1}^{-1})_{t_2,t_1} (\bGG_{\xi^{k,s(i)},t-1})_{t_2,t_3} 
    \rt)
    \diamond
    (\bZ)_{j,t_1}\, ,
%
\end{align}
%
Then $\hZZ_{k,t}$ is the unique solution of the following linear equation (with $\bY_{k,t}$ defined as per \eqref{eq:Ydef1})
%
\begin{align}
%
\hZZ_{k,t}+\cT_{k,t}(\hZZ_{k,t}) =\bY_{k,t}.\label{eq:ZZ-eq}
%
\end{align}

(Here, $\hZZ_{k,t} = [\hat{\bz}_{k,0},\cdots,\hat{\bz}_{k,t-1}]$ and $\bY_{k,t} = [\hat{\by}_{k,1},\cdots,\hat{\by}_{k,t}]$ have dimensions $N \times t$.)
%
\end{lemma}
%
%\am{Again, not clear the time index for $\bY_{k,t}$ is correct.}
%\ms{Right, changed}

The above formulas for $\E[\bA^{(k)}|\cF_t]$ and $\cT_{k,t}$ are rather complicated. In \cite[Appendix A]{ams20} the reader may find helpful tensor network diagrams for the single-species case. Unfortunately it is less clear how to draw a corresponding tensor network with multiple species.


\begin{proof}[Proof of Lemma \ref{lem:symregression}]
Let $\cV_{k,t}$ be the affine space of symmetric tensors satisfying the constraint \eqref{eq:LinearConstraint}.
The conditional expectation $\E[\bA^{(k)}|\cF_t]$ is the tensor with minimum weighted Frobenius norm $\|\cdot\|_{F,\xi^k}$ in the affine space $\cV_{k,t}$, given by
\begin{equation}
\label{eq:Gammak-inner-product}
    \|\bA\|_{F,\xi^k}^2
    =
    \langle 
    (\Gamma^{(k)})^{-1}\diamond \bA
    ,
    (\Gamma^{(k)})^{-1}\diamond\bA
    \rangle.
\end{equation}
Here $(\Gamma^{(k)})^{-1}$ is the entry-wise inverse of $\Gamma^{(k)}$, which exists by Assumption~\ref{as:degree-D}.

By Lagrange multipliers, there exist vectors $\bm_1,\dots,\bm_t\in\bbR^N$ such that $\E[\bA^{(k)}|\cF_t]=\hbA^{(k)}$ equals
%
\begin{align}
%
    \hbA^{(k)}_t \equiv\Gamma^{(k)}\diamond
    \sum_{t'=0}^{t-1}\sum_{j=1}^k \underbrace{\f_{t'}
    \otimes 
    \cdots 
    \otimes 
    \f_{t'}}_{\mbox{$j-1$ times}}\otimes\bm_{t'} 
    \otimes
    \underbrace{\f_{t'}\otimes \cdots \otimes \f_{t'}}_{\mbox{$k-j$ times}}\, .
%
\end{align}
%


Also by Lagrange multipliers, if a tensor $\hbA^{(k)}$ of this form (for some choice of vectors $\bm_1,\dots,\bm_t$) satisfies the constraints $\hbA^{(k)}\{\f_{t'}\}=\by_{k,t'+1}$
for $s< t$, then such a tensor is unique, and corresponds to $\E[\bA^{(k)}|\cF_t]$.
Without loss of generality, we write 
%
\begin{align}
%
\bm_r =  \sum_{t'=0}^{t-1}(\bG^{-1}_{\xi^{k,s},t-1})_{r,t'}\hbz_{t'}\, , \;\;\;\; \hZZ_{k,t}= [\hbz_1|\;\cdots\;|\hbz_t]\, .
%
\end{align}
%
By direct calculation we obtain that for each $i\in [N]$,
%
\begin{align}
\label{eq:SumT}
    \big(\hbA^{(k)}_t\{\f_{t_1}\}\big)_i &= \sum_{t_2=0}^{t-1} (\bG_{\xi^{k,s(i)},t-1})_{t_1,t_2}(\bm_{t_2})_i
    + 
    \sum_{t_2=0}^{t-1} (\bGG_{\xi^{k,s(i)},t-1})_{t_1,t_2}\<\f_{t_1},\bm_{t_2}\>(\f_{t_2})_i
    \\
    &= 
    (\hbz_{t_1})_i
    +
    \sum_{t_2=0}^{t-1} (\bGG_{\xi^{k,s(i)},t-1})_{t_1,t_2}\<\f_{t_1},\bm_{t_2}\>(\f_{t_2})_i
    \, .
%
\end{align}


We next stack these vectors as columns of an $N\times t$ matrix. The first term yields $\hZZ_{k,t}$. Moreover the second term
coincides with $\cT_{k,t}(\hZZ_{k,t})$ as following by rearranging the order of sums in \eqref{eq:SumT}. Hence
%
\begin{align}
%
    \big[\hbA^{(k)}_t\{\f_{0}\},\cdots,\hbA^{(k)}_t\{\f_{t-1}\}\big] 
    & =  
    \hZZ_{k,t} + \cT_{k,t}(\hZZ_{k,t})\, .
%
\end{align}
%
This in turn implies that the equation determining $\hZZ_{k,t}$ takes the form \eqref{eq:ZZ-eq}.
\end{proof}



\subsection{Long AMP}
\label{sec:LAMP}

As an intermediate step towards proving Theorem \ref{thm:mixedAMP}, we introduce a new iteration that we call Long AMP (LAMP), following 
\cite{berthier2019state}. This iteration is less compact but simpler to analyze. For each $k\le D$, let  
$\cS_{k,t}\subseteq (\bbR^N)^{\otimes k}$ be the linear subspace of tensors $\bT$ that are symmetric and such that
$\bT\{\f_{t_1}\}=0$ for all $t_1<t$.   We denote by $\cP_t^{\perp}(\bA^{(k)})$ the projection of $\bA^{(k)}$ 
onto $\cS_{k,t}$, in the inner product space \eqref{eq:Gammak-inner-product} corresponding to $\Gamma^{(k)}$. 
We then define the LAMP mapping 
%
\begin{align}
\label{eq:LAMP1}
    \LAMP_t\lt(\bv^{\le t}\rt)_{k}
    &\equiv
    \cP_t^{\perp} (\bA^{(k)})
    \{\f_t\}
    +
    \sum_{0\leq t_1\leq t}  
    h_{t,t_1-1,k}
    \diamond 
    \qq^{k,t_1},
    \\
\label{eq:LAMP2}
    h_{t,t_1,k,s}
    &\equiv 
    \sum_{0\le t_2\le t-1}
    \big[\bG_{\xi^{k,s},t-1}^{-1}\big]_{t_1,t_2}
    \big[\bG_{\xi^{k,s},t}\big]_{t_2,t}
    ,~~~ h_{t,-1,k}=0. 
\end{align}
%
Here we use similar notations $\f_t = f_t(\VV_t;\bE_t)$ and $\bG_{\xi^{k,s},t}$ as before (recall \eqref{eq:bG-def}), and take the vectors $\be^t$ as before. However the quantities $\f_t,\bG_{\xi^{k,s},t}$ are now different: they are computed using the vectors $\bv^0,\dots,\bv^t$ using the recursion:
\begin{align}
    \bv^t=\sum_{2\leq k\leq D} \qq^{k,t}\, ,\;\;\;\;\;\;\;
    \qq^{k,t+1}=\LAMP_t\lt(\bv^{\le t}\rt)_{k}\, . 
\end{align}


%
Following \cite{berthier2019state,ams20}, we first establish state evolution for LAMP (under the non-degeneracy Assumption~\ref{as:degree-D}), and then deduce the result for the original AMP.
In analyzing LAMP we use notations analogous to the ones introduced for AMP. In particular:
%
\begin{align}
    \VV_{t}
    &=
    [\bv_{1}|\bv_{2}|\dots|\bv_{t}]
    \\
    \bQ_{k,t}
    &=
    [
    \qq_{k,1}^{\otimes k}|
    \qq_{k,2}^{\otimes k}|
    \dots|
    \qq_{k,t}^{\otimes k}
    ].
\end{align}
%


\subsection{State Evolution for Long AMP}
 
%
\begin{theorem}
\label{thm:SELAMP}
  Under the assumptions of Theorem \ref{thm:mixedAMP}, let $\qq^{2,0},\cdots \qq^{D,0}\in\bbR^N$
be deterministic vectors and $\bv^0 =\sum_{2\leq k\leq D} \bq^{k,0}$.
Assume that the uniform empirical distribution of the $N$ vectors $\{(q_i^{2,0},\cdots, q_i^{D,0})\}_{i\leq N}$ converges 
in $\bbW_2$ distance to the law of the vector $(U^{k,0})_{2\le k\le D}$.

Further we assume there is a constant $C<\infty$ such that for all $t\le T$:
%
\begin{itemize}
%
\item[$(i)$] The matrices $\bG_{\xi^{k,s},t}= \bG_{\xi^{k,s},t}(\VV)$ are uniformly well-conditioned as guaranteed by Assumption~\ref{as:well-conditioned}.
%
\item[$(ii)$] Let the linear operator $\cT_{k,t}:\bbR^{N\times t}\to\bbR^{N\times t}$ be defined as per \eqref{eq:Tdef}, with $\bG_{\xi^{k,s},t} = \bG_{\xi^{k,s},t}(\VV,\bE)$,
and  $\f_t=f_t(\VV,\bE)$, and define 
\begin{equation}
\label{eq:cL-k-t}
\cL_{k,t} = {\boldsymbol 1}+\cT_{k,t}.
\end{equation}
Then $C^{-1}\le \sigma_{\min}(\cL_{k,t})\le \sigma_{\max}(\cL_{k,t})\le C$.
%
\end{itemize}

Then the following statements hold for any $t\le T$ and sufficiently large $N$:
%
\begin{enumerate}[label=(\alph*)]
\item Correct conditional law: 
%
\begin{equation}\label{eq:conditional}
%
\qq^{k,t+1}|_{\mathcal F_t}\ed \E[\qq^{k,t+1}|\mathcal F_t] +  \cP_t^{\perp}(\tbA^{(k)}) \{\f_t\}\, .
%
\end{equation}
%
where $\tbA^{(k)}$ is a symmetric tensor distributed identically to $\bA^{(k)}$ and independent of everything else,  and
$\cP_{t}^{\perp}$ is the projection onto the subspace $\cS_{k,t}$ defined in Section \ref{sec:LAMP}.
Further 
\begin{equation}
\label{eq:CondExp}
    \E[\qq^{k,t+1}|\mathcal F_t]
    = 
    \sum_{s\in\sS}
    \sum_{0\leq t_1\leq t}  
    h_{t,t_1-1,k,s}
    \qq^{k,t_1}_s\, .
\end{equation}
%
Moreover, the vectors $(\qq^{k,t+1})_{2\leq k\leq D}$ are conditionally independent given $\mathcal F_t$. 
%
\item Approximate isometry: we have
 %   
\begin{align}
\label{eq:c1}
    R_s(\qq^{k,t_1+1},\qq^{k,t_2+1})
    &\simeq 
    \xi^{k,s}\lt(\vR( \f_{t_1},\f_{t_2})\rt)\, ,
    \\
\label{eq:c3}
    R_s(\bv^{t_1+1},\bv^{t_2+1})
    &\simeq 
    \xi^{s}\big(\vR( \f_{t_1},\f_{t_2})\big). 
\end{align}
%
Moreover, both sides converge in probability to constants as $N\to\infty$, and for $k_1\neq k_2$ and any $(t_1,t_2)$ and $s\in\sS$,    
\begin{equation}
\label{eq:c2}
    R_s(\qq^{k_1,t_1},\qq^{k_2,t_2})\simeq 0.
\end{equation}
%
\item  State evolution: for each $s\in\sS$ and any pseudo-Lipschitz function 
$\psi:\bbR^{D \times 2(t+1)}\to \bbR$, we have
%
\begin{align}
\label{eq:ConvergenceLAMP}
    \plim_{N\to\infty}
    \frac{1}{N_s}
    \sum_{i\in\cI_s}
    \psi\big((q_i^{k,t'})_{ k\le D,t'\le t}; (e^t_i)_{t'\leq t}\big) 
    = 
    \E\big\{\psi\big((U^{k,t'}_s)_{2\leq k\leq D,t'\leq t}; 
    (E^{t'}_s)_{t'\leq t}
    \big)\big\}\, .
%
\end{align}
%
where $(U^{k,t}_s)_{k\le D,1\le t\le T}$ is the centered Gaussian process defined in the statement of  Theorem \ref{thm:mixedAMP}.
\end{enumerate}
\end{theorem}
% %
% %
In the next subsection, we will prove these statements by induction on $t$. The crucial point we exploit is the representation $(a)$. We emphasize that the iteration number $t$ is bounded as $N\to\infty$; therefore all numerical quantities not depending on $N$ (but possibly on $t$) will be treated as constants. 


\subsection{Proof of Theorem~\ref{thm:SELAMP}}

The proof will be by induction over $t$. The base case is clear, so we focus on the inductive step. We assume the statements above for $t-1$ and prove them for $t$. 

\subsubsection{Proof of $(a)$}

Note that $\cP_t^{\perp}(\bA^{(k)})$ is by construction independent of $\cF_t$, and therefore we can replace $\bA^{(k)}$
by a fresh independent matrix in \eqref{eq:LAMP1}, whence \eqref{eq:conditional} follows. The equality \eqref{eq:CondExp} holds by definition of the iteration.


\subsubsection{Proof of $(b)$: Approximate isometry}

We will repeatedly apply Lemma~\ref{lem:4}. We start with  \eqref{eq:c1}. As we are inducting on $t$, we may limit ourselves to considering overlaps
$\vR( \qq^{k,t+1},\qq^{k,t_1+1})$, for $t_1\le t$. 

Define the tensor $\Gamma^{(k),\nabla}\in (\bbR^{\sS}_{\geq 0})^{\otimes (k-1)}$ by
\begin{equation}
\label{eq:Gamma-nabla-def}
    \Gamma^{(k),\nabla}_{s_1,\dots,s_{k-1}}
    =
    \sqrt{
    k
    \sum_{s\in\sS}
    \lambda_s
    \big(\Gamma^{(k)}_{s,s_1,\dots,s_{k-1}}\big)^2
    }.
\end{equation}
We choose 
\[
    (\f_{t}^{\otimes k-1})_{\parallel}
    \in
    {\rm span}\lt(\f_{t_1}^{\otimes k-1}\rt)_{t_1< t}
\]
such that
\[
    \Gamma^{(k),\nabla}\diamond \big(\f_{t}^{\otimes k-1}\big)_{\parallel}
\]
is the orthogonal projection of $\Gamma^{(k),\nabla}\diamond \f_{t}^{\otimes k-1}$ onto 
\[
    {\rm span}\lt(\Gamma^{(k),\nabla}\diamond\f_{t_1}^{\otimes k-1}\rt)_{t_1< t}
\]
and also set
\[
    (\f_{t}^{\otimes k-1})_{\perp}=\f_{t}^{\otimes k-1}-(\f_{t}^{\otimes k-1})_{\parallel}.
\]

We will use (and soon after, prove) the following lemma.
\begin{lemma}
\label{lem:LemmaPerp}
For all $t_1\leq t_1$, we have
\begin{equation}
\label{eq:LemmaPerp2}
    \cP_t^{\perp} (\tbA^{(k)})\{(\f_t^{\otimes k-1})_{\perp}\} \simeq
    \tbA^{(k)}\{(\f_t^{\otimes k-1})_{\perp}\}\, .
\end{equation}
\end{lemma}
%
For $t_1\le t-1$, using Lemma~\ref{lem:4}, point 2 implies
\begin{align*}
    \vR(\qq^{k,t+1},\qq^{k,t_1+1}) 
    \simeq 
    \vR\big(\E[\qq^{k,t+1}|\cF_t],\, \qq^{k,t_1+1}\big)
\end{align*}
%
We next use the formula in $(a)$ for $\E[\qq^{k,t+1}|\cF_t]$ together with the expression in \eqref{eq:LAMP1}. For each $s\in\sS$:
\begin{align}
\nonumber
    R\big(\mathbb E[\qq^{k,t+1}|\mathcal F_t],\qq^{k,t_1+1}\big)_s
    &\simeq
    R\Bigg(
    \sum_{0\leq t_2,t_3\leq t-1}
    \qq^{k,t_3+1}(\bG_{\xi^{k,s},t-1}^{-1})_{t_3,t_2}
    \,
    \xi^{k,s}\big(\f_{t_2},\f_{t}\big)
    ,\, \qq^{k,t_1+1}
    \Bigg)_s
    \\
\nonumber
    &= 
     \sum_{0\leq t_2,t_3\leq t-1}
     R\big(\qq^{k,t_3+1},\qq^{k,t_1+1}\big)_s
     \,
     (\bG_{\xi^{k,s},t-1}^{-1})_{t_3,t_2} 
     \,
     \xi^{k,s}\big(\f_{t_2},\f_{t}\big)
    \\
\label{eq:3rd-ineq}
    &\simeq
    \sum_{0\leq t_2,t_3\leq t-1} 
    (\bG_{\xi^{k,s},t-1})_{t_3,t_1}
    \,
    (\bG_{\xi^{k,s},t-1}^{-1})_{t_3,t_2} 
    \,
    \xi^{k,s}\big(\f_{t_2},\f_{t}\big)
    \\
\nonumber
    &=
    \big(
    \bG_{\xi^{k,s},t-1}
    \times 
    \bG_{\xi^{k,s},t-1}^{-1}
    \times
    \bG_{\xi^{k,s},t-1}
    \big)_{t_1,t}
    \\
\nonumber
    &=
    (\bG_{\xi^{k,s},t-1})_{t_1,t}.
%
\end{align}
Here \eqref{eq:3rd-ineq} comes from the induction hypothesis \eqref{eq:c1} (and the symmetry of the matrix $\bG_{\xi^{k,s},t-1}$ is used to obtain the next line). We next prove that \eqref{eq:c1} holds for $t_1=t$. We have by definition of the projections that
%
\begin{align*}
\cP_t^{\perp} (\tbA^{(k)})\{\f_t\}=\cP_t^{\perp} (\tbA^{(k)})\{(\f_t^{\otimes k-1})_{\perp}\} \, ,
\end{align*}
%
where the right-hand side is defined according to \eqref{eq:TensorTensor}.
%
Using \eqref{eq:LemmaPerp2} from Lemma~\ref{lem:LemmaPerp} as well as point~4 of Lemma~\ref{lem:4}, we have
%
\begin{align}
\label{eq:PAnorm}
    R\lt(
    \cP_t^{\perp} (\tbA^{(k)})\{\f_t\}
    \,,
    \cP_t^{\perp} (\tbA^{(k)})\{\f_t\}
    \rt)_s
    \simeq 
    \xi^{(k,s)}\lt(
    R\big(
    (\f_{t}^{\otimes k-1})_{\perp}
    \,,
    (\f_{t}^{\otimes k-1})_{\perp}
    \big)
    \rt).
\end{align}
%
Next, using \eqref{eq:LemmaPerp2} and Lemma~\ref{lem:4} (point 2), we obtain that for all $s\in\sS$
%
\begin{equation}
\label{eq:ApproxOrth}
    R\big(\cP_t^{\perp} (\tbA^{(k)})\{\f_t\},\E[\qq^{k,t+1}|\cF_t]\big)_s \simeq 0\, .
\end{equation}
%
Moreover we recall that by the expression for $\E[\qq^{k,t+1}|\cF_t]$ from part $(a)$,
%
\begin{align}
%
    R\lt(
    \E[\qq^{k,t+1}|\mathcal F_t]
    \,,
    \E[\qq^{k,t+1}|\mathcal F_t]
    \rt)
    \simeq
    \xi^{k,s}
    \lt(
    \vR(
    (\f_t^{\otimes k-1})_{\parallel}
    \,,
    (\f_t^{\otimes k-1})_{\parallel}
    )
    \rt).
%
\end{align}
%
The formula for linear regression implies
%
\begin{align}
\label{eq:lin-reg-1}
%
    (\f_{t}^{\otimes k-1})_{\parallel}
    & =
    \sum_{0\leq t_1\leq t-1} \alpha_{t_1,t} \Gamma^{(k,s)}\diamond \f_{t_1}^{\otimes k-1},
    \\
    \alpha_{t_1,t}
    &=
    \sum_{0\leq t_2\le t-1} 
    (\bG_{\xi^{k,s},t-1}^{-1})_{t_1,t_2}
    \< 
    \Gamma^{(k,s)}\diamond \f_{t_2}^{\otimes k-1},
    \Gamma^{(k,s)}\diamond \f_{t}^{\otimes k-1}
    \>_N
    \\
    &=
    \sum_{0\leq t_2\le t-1} 
    (\bG_{\xi^{k,s},t-1}^{-1})_{t_1,t_2}
   (\bG_{\xi^{k,s},t}^{-1})_{t_2,t}
    \, .
%
 \end{align}
%

By part $(b)$ of the inductive step, for $1\leq t_1,t_2\leq t-1$ we have
\[
    \xi^{k,s}\big(\vR( \f_{t_2},\f_{t_1})\big)
    \simeq 
    R_s( \qq_{k,t_2+1},\qq_{k,t_1+1})
    \,.
\]
In particular the formulas \eqref{eq:LAMP2} and \eqref{eq:lin-reg-1} have asymptotically the same coefficients, and the overlap structure between the summands is identical. It follows that
\begin{align}
\label{eq:CEnorm}
    R\lt(
    \E[\qq^{k,t+1}|\mathcal F_t],
    \,,
    \E[\qq^{k,t+1}|\mathcal F_t]
    \rt)
    \simeq
    R\lt(
    (\f_{t}^{\otimes k-1})_{\parallel}
    \,,
    (\f_{t}^{\otimes k-1})_{\parallel}
    \rt).
\end{align}
%
Using together Eqs.~\eqref{eq:PAnorm}, \eqref{eq:ApproxOrth}, and \eqref{eq:CEnorm}, we get
%
\begin{align*}
%
    R\lt(\qq^{k,t+1},\qq^{k,t+1}\rt)
    &\simeq 
    R\lt(\E[\qq^{k,t+1}|\mathcal F_t]
    \,,
    \E[\qq^{k,t+1}|\mathcal F_t]
    \rt)
    + 
    R\lt(
    (\f_t^{\otimes k-1})_{\perp}
    \,,
    (\f_t^{\otimes k-1})_{\perp}
    \rt)
    \\
    &\simeq
    R\lt(
    (\f_t^{\otimes k-1})_{\perp}
    \,,
    (\f_t^{\otimes k-1})_{\perp}
    \rt)
    \\
    &=
    \xi^{k,s}\lt(
    \vR( \f_t,\f_t)
    \rt)
    \,.
%
 \end{align*}
%
This establishes \eqref{eq:c1}.

Next consider \eqref{eq:c2}, i.e., approximate orthogonality of $\qq^{k,r}$ and $\qq^{p',r}$ for $k\neq p'.$ This follows easily from the representation
in point $(a)$ which, together with Lemma~\ref{lem:4}, inductively implies that the iterates $\qq^{s,k}$ for different $k$ are approximately orthogonal.
Finally, \eqref{eq:c3}  follows directly from \eqref{eq:c1} and \eqref{eq:c2}.
We now prove Lemma~\ref{lem:LemmaPerp}.

\begin{proof}[Proof of Lemma~\ref{lem:LemmaPerp}]
For convenience we write $\tbA=\tbA^{(k)}$. By Lagrange multipliers, there exist vectors
    $(\btheta_{t_1})_{t_1 \le t-1}$ in $\bbR^N$ such that $\cP_t^{\perp} (\tbA) = \tbA - \bQ$, where 
\begin{align*}
  \bQ = 
  \big(\Gamma^{(k)}\big)^{\odot 2}
  \diamond
  \frac{(k-1)!}{N^{k-1}}\sum_{t_1=0}^{t-1} \sum_{j=1}^k  \underbrace{\f_{t_1}\otimes \cdots \otimes \f_{t_1}}_{\mbox{$j-1$ times}}\otimes \btheta_{t_1} \otimes \underbrace{\f_{t_1}\otimes \cdots \otimes \f_{t_1}}_{\mbox{$k-j$ times}}.
\end{align*}
%
The vectors $(\btheta_{t_1})_{t_1 \le t-1}$ are determined by the equations
% $\cP_t^{\perp} (\tbA) \{\f_{t_1}\} = 0$
$\bQ \{\f_{t_1}\}=\tbA \{\f_{t_1}\}$
for all $t_1\le t-1$.
This expands (for each $t_1\leq t-1$) to
%
\begin{align*}
  %
  \sum_{t_2\leq t-1} 
  (\bG_{\xi^{k,s},t-1})_{t_1,t_2}
  \diamond 
  \btheta_{t_2}
  +
%   (k-1)
  \sum_{t_2\leq t-1}
  (\bGG_{\xi^{k,s}})_{t_1,t_2}
  \diamond
  \<\f_{t_1},\btheta_{t_2}\>_N \f_{t_2}
  = 
  \tbA\{\f_{t_1}\}\, .
  %
\end{align*}
%
Recall that we assume each $\bG_{\xi^{k,s},t-1}$ is well conditioned with high probability. Thus we can multiply the system of $t$ equations above by $\bG_{\xi^{k,s},t-1}^{-1}$ in the coordinates $\cI_s$ for each $s\in\sS$. For each $t_3\leq t-1$, we obtain:
%
\begin{align}
\label{eq:LambdaEq}
  \btheta_{t_3}
  +
  \sum_{t_1,t_2<t}
  \lt(
  (\bG_{\xi^{k,s},t-1}^{-1})_{t_1,t_3} (\bGG_{\xi^{k,s},t-1})_{t_1,t_2}
  \rt)
  \diamond
  \<\f_{t_1},\btheta_{t_2}\>_N \f_{t_2}=
  \sum_{t_1<t}
  (\bG_{\xi^{k,s},t-1}^{-1})_{t_1,t_3}
  \diamond
  \tbA\{\f_{t_1}\}\, . 
  %
\end{align}
%
Switching $t_3$ to $t_1$, we find
%
\begin{align}
\nonumber
  %
  \btheta_{t_1} &=   \btheta^0_{t_1}+ \btheta^{\parallel}_{t_1}\, ,
  \\
\label{eq:theta0}
  \btheta^0_{t_1}
  &\equiv
  \sum_{t_2<t}
  (\bG_{\xi^{k,s},t-1}^{-1})_{t_1,t_2}\diamond \tbA\{\f_{t_2}\} \, ,
  \\
\nonumber
  \btheta^{\parallel}_{t_1}
  &\in 
  \spn\lt((\f_{t_2,s})_{t_2<t,s\in\sS}\rt).
  %
\end{align}
%
We claim that $\|\btheta^{\parallel}_{t_1}\|_N\simeq 0$, i.e.,
$\btheta_{t_1}\simeq   \btheta^0_{t_1}$. Indeed, let $\bTheta\in\bbR^{N\times t}$ be the matrix with columns
$(\btheta_{t_2})_{t_2<t}$, and $\bTheta^0$ the matrix with columns $(\btheta^0_{t_2})_{t_2<t}$.
Then \eqref{eq:LambdaEq} can be written as
%
\begin{align*}
  %
  \cL_{k,t}^{\sT}(\bTheta) =\bTheta^0\, .
  %
\end{align*}
%
Here we recall $\cL_{k,t}=\bfone+\cT_{k,t}$ and $\cT_{k,t}\in\bbR^{Nt\times Nt}$ is defined in \eqref{eq:Tdef}.
Substituting the decomposition 
$\bTheta = \bTheta^0+\bTheta^{\parallel}$ in the above, we obtain
%
\begin{align*}
  %
  \cL_{k,t}^{\sT}(\bTheta^{\parallel}) =-\cT^{\sT}_{k,t}(\bTheta^0)\, .
  %
\end{align*}
%
Recall that $\cL_{k,t}$ is well conditioned by Assumption~\ref{as:well-conditioned}. Therefore it remains to prove 
\begin{equation}
\label{eq:key-lamp-computation}
    \cT^{\sT}_{k,t}(\bTheta^0)\stackrel{?}{\simeq} 0.
\end{equation}
%
Let $\bc_0,\cdots,\bc_{t-1} \in \bbR^N$ be the columns of $\cT^{\sT}_{k,t}(\bTheta^0)$. We first note that for all $t_1\leq t-1$ and $s\in\sS$, 
\[
    \bc_{t_1,s} \in \spn((\f_{t_2,s})_{t_2<t}).
\]
Moreover the Gram matrix 
\[
    \bG_{1,t-1,s}=\lt(R_s(\f_{t_1},\f_{t_2})\rt)_{t_1,t_2<t}
\]
is well conditioned for each $s\in\sS$. Therefore it is sufficient to check that $R_s(\f_{t_1},\bc_{t_4})\simeq 0$ for each $t_1,t_4<t$ and $s\in\sS$. Plugging in the definition \eqref{eq:Tdef}, it remains to check
%
\begin{align*}
  \sum_{t_2,t_3<t}
  \lt\<
  \f_{t_1}
  ,
  \,
  (\bG_{\xi^{k,s},t-1}^{-1})_{t_2,t_3} 
  (\bGG_{\xi^{k,s},t-1})_{t_4,t_3}
  \diamond
  \btheta^0_{t_2}
  \rt\>_N 
  R_s(\f_{t_1},\f_{t_3})
  \stackrel{?}{\simeq} 
  0\, 
  ,
  \quad
  \forall~ 0\leq t_1,t_4\leq t-1\,.
\end{align*}
%
Finally, this last claim follows by substituting the definition \eqref{eq:theta0} of $\btheta^0_{t_2}$, and using the fact that  
\[
    R_s(\f_{t_1},\tbA\{\f_{t_3}\})\simeq 0,\quad
    \forall~ t_1,t_3\le t,\,s\in\sS
\]
which follows from Lemma \ref{lem:4}. Thus \eqref{eq:key-lamp-computation} is established.



We are now ready to prove Lemma~\ref{lem:LemmaPerp}. 
First note that 
\begin{equation}
\label{eq:god}
     \tbA\{(\f_t^{\otimes k-1})_{\perp}\} 
    -
    \cP_t^{\perp} 
    (\tbA)
    \{(\f_t^{\otimes k-1})_{\perp}\} 
    = 
    \bQ\{(\f_t^{\otimes k-1})_{\perp}\}
\end{equation}
decomposes into two types of terms based on the definition of $\bQ$ above. Recalling \eqref{eq:Gamma-nabla-def}, the first involves
\[
    \lt\langle 
    \Gamma^{(k),\nabla}
    \diamond 
    (\f_{t_1}^{\otimes k-1})_{\perp}
    ,
    \Gamma^{(k),\nabla}
    \diamond 
    (\f_t^{\otimes k-1})_{\perp}
    \rt\rangle_N
    \btheta_{t_1}
\]
for $t_1\leq t-1$, which vanishes by the definition of $(\f_t^{\otimes k-1})_{\perp}$. The other terms take the form
\[
    \lt\langle 
    \Gamma^{(k),\nabla}
    \diamond 
    (\btheta_{t_1}\otimes \f_{t_1}^{\otimes k-2})
    ,\,
    \Gamma^{(k),\nabla}
    \diamond 
    (\f_t^{\otimes k-1})_{\perp}
    \rt\rangle_N
    ~
    \f_{t_1}.
\]
In particular, this means that to prove \eqref{eq:god} vanishes, suffices to show
\[
    R\lt(
    \bQ\{(\f_t^{\otimes k-1})_{\perp}\}
    ,\,
    \f_{t_2}
    \rt)
    =0
\]
for all $t_2\leq t$.


Note that by construction,
\[
   (\f_t^{\otimes k-1})_{\perp}
   =
   \sum_{t_1\leq  t} b_{t_1} \f_{t_1}^{\otimes k-1}
    \,.
\]
By the well-conditioning assumption, the $b_{t_1}$ are bounded. Therefore it suffices to show that 
\[
    R\lt(
    \bQ\{\f_{t_2}^{\otimes k-1}\}
    ,\,
    \f_{t_1}
    \rt)
    \stackrel{?}{\simeq} 
    0,
    \quad 
    \forall\, t_1\leq t-1,\,t_2\leq t.
\]
Finally note that each term in the left-hand side includes an overlap $R_s(\btheta_{t_1},\f_{t_2})$. However these all vanish:
\[
    R_s(\btheta_{t_1},\f_{t_2})
    \simeq
    0.
\]
This is because we can substitute $\btheta_{t_1}$ with $\btheta_{t_1}^0$ as defined in \eqref{eq:theta0} and use the fact that $\vR(\tbA\{\f_{t_3}\},\f_t)\simeq 0$ which follows from Lemma \ref{lem:4}. This completes the proof.
\end{proof}


\subsubsection{Proof of $(c)$}

Recall that the process $(U^{k,t}_s)_{t\ge 1}$ is Gaussian by construction, and independent of $U^{k,0}_s$. Define 
\begin{align*}
    C_{t_1,t_2,s} &= \E\big[U^{k,t_1}_s U^{k,t_2}_s\big]\,;
    \\
    \bC_{\le t,s} &= (C_{t_1,t_2,s})_{t_1,t_2\le t}\,.
\end{align*}
We then have
%
\begin{equation} 
\label{eq:wt-alpha}
\begin{aligned}
    \E[U^{k,t+1}_s| U^{k,0}_s,\dots,U^{k,t}_s]
    &=
    \sum_{t_1=1}^t 
    \wt\alpha_{t_1,s} U^{k,t_1}
    \, ;
    \\
    \wt\alpha_{t_1,s}
    & \equiv
    \sum_{t_2=1}^t
    (\bC^{-1}_{\le t,s})_{t_1,t_2}C_{t_2,t+1,s}
    \, .
\end{aligned}
\end{equation} 
Here in writing $(\bC^{-1}_{\le t,s})_{t_1,t_2}$, we view $\bC_{\le t,s}$ as a $(t+1)\times (t+1)$ matrix for each $s\in\sS$.
%

On the other hand, from point $(a)$, we know that
%
\begin{equation} 
\label{eq:alpha}
\begin{aligned}
    \E[\qq^{k,t+1}_{s}|\mathcal F_t]
    & = 
    \sum_{1\leq t_1\leq t}  
    \alpha_{t_1,s} 
    \qq^{t_1,k}_s\, ;
    \\
    \alpha_{t_1,s}
    & \equiv
    \sum_{t_2=1}^t
    (\bG^{-1}_{\xi^{k,s},t-1})_{t_1-1,t_2-1} 
    (\bG_{\xi^{k,s},t})_{t_2-1,t}
    \, .
\end{aligned}
\end{equation} 
%
Moreover the induction hypothesis of \eqref{eq:ConvergenceLAMP} implies that for $t_1,t_2 \le t$,
%
\begin{equation}
\label{eq:augment-e-for-W2}
    (\bG_{\xi^{k,s},t})_{t_1,t_2} 
    \simeq 
    \bbE\lt[
    \xi^{k,s}
    \lt(
    f_{t_1}(W^0_s,\dots,W^{t_1}_s;E^0_s,\dots,E^{t_1}_s), f_{t}(W^0_s,\dots,W^{t_2}_s;E^0_s,\dots,E^{t_2}_s)\}
    \rt)
    \rt]
    \, .
\end{equation}
%
(Recall that by definition $W^t_s \equiv \sum_{k\le D} U^{k,t}_s$, while $\f_t=f_t(\VV_t;\bE_t)$ here.) 


Therefore, from the definition of the process $(U^{k,t}_s)_{t\ge 0}$,
\[
    (\bG_{\xi^{k,s},t})_{t_1,t_2} \simeq C_{t_1+1,t_2+1,s}
    ,
    \quad\quad \forall t_1,t_2\le t.
\]
Recalling that $\bG_{\xi^{k,s},t}$ is well conditioned, we find (recall \eqref{eq:wt-alpha},\eqref{eq:alpha}):
\[
    \alpha_{t_1,s}\simeq \wt\alpha_{t_1,s}.
\]
Therefore we also have 
%
\begin{align*}
    \E[\qq^{k,t+1}|\mathcal F_t] - \sum_{t_1=1}^t \wt\alpha_{t_1}\diamond \qq^{k,t_1}
    &=
    \sum_{t_1=1}^t (\alpha_{t_1}-\wt\alpha_{t_1}) \diamond \qq^{k,t_1}
    \\
    &\simeq 
    0.
%
\end{align*}
%
Moreover, Lemma~\ref{lem:4} (point 4) shows that $\cP^{\perp}_t(\tbA^{(k)})\{\f_t\}\simeq\tbA^{(k)}\{(\f_{t}^{\otimes k-1})_{\perp}\}$ 
has entries which are approximately independent Gaussian with variance 
\[
    \sigma^2_{t,s}\equiv 
    \lt(
    \Gamma^{(k),\nabla}
    \diamond
    (\f_{t}^{\otimes k-1})_{\perp}
    ,\,
    \Gamma^{(k),\nabla}
    \diamond
    (\f_{t}^{\otimes k-1})_{\perp}
    \rt)
\]
on coordinates $i\in\cI_s$, even conditionally on $\cF_t$. 
Therefore
%
\begin{align}
\label{eq:ReprSE}
  %
  \qq^{k,t+1} &\ed \sum_{t_1=1}^t \wt\alpha_{t_1} \diamond\qq^{k,t_1} +\sigma_t \diamond \bg + \bferr^{k,t+1}\, ,
  %
\end{align}
%
where $\|\bferr\|_N\simeq 0$ and $\bg\sim\normal(\bfzero,\id_N)$ is independent of everything else.
It now remains to verify that this agrees with the desired covariance.
As proved in the previous point, for any $t_1\le t$,
%
\begin{align*}
  %
  R\lt(\qq^{k,t+1} ,\qq^{k,t'+1}\rt)_s
  &\simeq 
  \xi^{k,s}\lt(
  \f_t,\f_{t'}
  \rt)
  \\
  &\simeq
  \E\big[ 
  U^{k,t+1}_s U^{k,t'+1}_s
  \big]\, .
%
\end{align*}
%
Therefore, in order to  prove \eqref{eq:ConvergenceLAMP}, it is sufficient to consider $\psi:\bbR^{D \times (t+1)}\to\bbR$  Lipschitz.
Using the representation \eqref{eq:ReprSE}, and focusing for simplicity on a single $k$, we get
%
\begin{align*}
  %
  \frac{1}{N_s}
  \sum_{i\in\cI_s}
  \psi\big(\qq_i^{k,\le t}, q_i^{k,t+1}
  ;
  \be^{\leq t}_i
  \big) 
  &\simeq 
  \frac{1}{N_s}
  \sum_{i\in\cI_s}
  \psi\lt(
      \qq_i^{k,\le t},
      \sum_{s=1}^t 
      \wt\alpha_s \qq^{k,s} 
      +
      \sigma_tg_i
      ;
    \be^{\leq t}_i
  \rt)
  \\
  &\simeq 
  \frac{1}{N_s}
  \sum_{i\in\cI_s}
  \bbE^{g\sim\cN(0,1)}
  \psi\lt(
  \qq_i^{k,\le t},
  \sum_{s=1}^t 
  \wt\alpha_s 
  \qq^{k,s} 
  +
  \sigma_t g
  ;
  \be^{\leq t}_i
  \rt)
  \, .
  %
\end{align*}
%
The second equality above follows by Gaussian concentration. Applying induction hypothesis now implies \eqref{eq:ConvergenceLAMP}, except that $\be^{t+1}$ is not present. 
However since $\be^{t+1}_i$ and $E^{t+1}_s$ have the same law and are both independent of the past, $\bbW_2$ convergence immediately transfers (this is the only step of the proof that involves the vectors $\be^t$ at all). This completes the proof.


\subsection{Asymptotic Equivalence of AMP and Long AMP}

Here we show that AMP and LAMP produce approximately the same iterates. 
%
\begin{lemma}
\label{lem:ampequalslamp}
Let $\{\bG^{(k)}\}_{k\le D}$ be standard Gaussian tensors, and $\bA^{(k)} = \Gamma^{(k)}\diamond \bG^{(k)}$ for $k\ge 2$. Consider the corresponding AMP
iterates $\ZZ_{t}\equiv (\bz^{k,t_1})_{k\le D,t_1\le t}$ and LAMP iterates $\bQ_{t}\equiv (\qq^{k,t_1})_{k\le D,t_1\le t}$,
from the same initialization $\ZZ_0=\bQ_0$ satisfying the assumptions of Theorem \ref{thm:mixedAMP}
and Theorem \ref{thm:SELAMP}.

Let $\f_t = f_t(\VV_t;\bE_t)$, $t\ge 0$ be the nonlinearities applied to LAMP iterates.
% and $(\bG_{k,t}(\VV))_{r,s}=\<\f_t,\f_{t'}\>^k$ be the corresponding Gram matrices.
Further assume that there exists a constant $C<\infty$ such that, for all $t\le T$,
%
\begin{itemize}
%
\item[$(i)$] The LAMP Gram matrices $\bG_{k,t} = \bG_{k,t}$ are
  well-conditioned as guaranteed by Assumption~\ref{as:well-conditioned}, i.e., 
 \[
    C^{-1}\le \sigma_{\min}(\bG_{k,t})\le \sigma_{\max}(\bG_{k,t})\le C,
    \quad\quad
    \forall k\le D,~t\le T\,.
\]
%
\item[$(ii)$] Let the linear operator $\cT_{k,t}:\bbR^{N\times t}\to\bbR^{N\times t}$ be defined as per \eqref{eq:Tdef}, with $\bG_{k,t} = \bG_{k,t}(\VV)$,
and $\f_t=f_t(\VV,\bE_t)$, and define $\cL_{k,t} = \bone+\cT_{k,t}$. Then 
\[
    C^{-1}\le \sigma_{\min}(\cL_{k,t})\le \sigma_{\max}(\cL_{k,t})\le C.
\]
%
\end{itemize}
%
Then, for any $t\le T$, we have
%
\begin{align}
%
\|\ZZ_{t} - \bQ_{t}\|_N\simeq 0 \, .
%
\end{align}
%
\end{lemma}
%
\begin{proof}
Throughout the proof we will suppress $\bE_t$ and simply write $f_t(\bW_t)$ or $f_t(\bV_t)$ to distinguish AMP and LAMP iterates, and analogously for
$\bG_{k,t}(\bW_t)$ or $\bG_{k,t}(\bV_t)$.
The proof is by induction over the iteration number, so we will assume it to hold at iteration $t$, 
and prove it for iteration  $t+1$. We prove the induction step by establishing the following two facts for each $2\leq k\leq D$:
%
\begin{align}
%
\big\|\AMP_{t+1}(\ZZ_{t})_k -\AMP_{t+1}(\bQ_{t})_k \big\|_N&\simeq 0 \, ,\label{eq:LAMPapprox1}\\
%
\big\|\AMP_{t+1}(\bQ_{t})_k -\LAMP_{t+1}(\bQ_{t})_k \big\|_N &\simeq 0\, . \label{eq:LAMPapprox2}
%
\end{align}

Let us first consider the claim \eqref{eq:LAMPapprox1}, and note that
%
\begin{align*}
    \AMP_{t+1}(\ZZ_{t})_k -\AMP_{t+1}(\bQ_{t})_k  &= \bA^{(k)}\{f_t(\bW_t)\}-\bA^{(k)}\{f_t(\bV_t)\} 
    \\
    &\quad - 
    \sum_{t_1\leq t} 
    d_{t,t_1,k}
    \diamond
    \big(f_{t_1-1}(\bW_{t_1-1})-f_{t_1-1}(\bV_{t_1-1})\big)\, ,
\end{align*}
%
where we wrote $d_{t,t_1,k,s}$ for the coefficients of \eqref{eq:AMP-def2}, with AMP iterates replaced by LAMP iterates. 
We then have 
%
\begin{align*}
%
    \big\|\AMP_{t+1}(\ZZ_{t})_k -\AMP_{t+1}(\bQ_{t})_k \big\|_N 
    &\le 
    D_{1,t}+D_{2,t}\, ;
    \\
    D_{1,t} 
    & \equiv 
    \big\| \bA^{(k)}\{f_t(\bW_t)\}-\bA^{(k)}\{f_t(\bV_t)\}\big\|_N\, ,
    \\
    D_{2,t} 
    &\equiv 
    \sum_{t_1\leq t,~s\in\sS} 
    |d_{t,t_1,k,s}| 
    \cdot 
    \big\|f_{t_1-1,s}(\bW_{t_1-1})- f_{t_1-1,s}(\bV_{t_1-1})\big\|_N\, .
%
\end{align*}
%
Notice that, by the induction assumption (and recalling that each $f_{t,s}$ is Lipschitz continuous and acts component-wise): 
%
\begin{equation}
\label{eq:InductionF}
%
    \big\|f_t(\bW_t)-f_t(\bV_t)\big\|_N
    \le C_T
    \sum_{t_1\le t,~k\le D}\|\bw^{k,t_1}-\bv^{k,t_1}\|_N 
    \simeq 
    0
    \, .
%
\end{equation}
%
Further, for any tensor $\bT\in(\bbR^{N})^{\otimes k}$, and any vectors $\bv_1,bv_2\in\bbR^N$,
%
\begin{align}
%
\|\bT\{\bv_1\}-\bT\{\bv_{2}\}\|_N\le (N^{\frac{k-2}{2}}\|\bT\|_{\op})  (\|\bv_1\|_N+\|\bv_2\|_N)^{k-2} \|\bv_1-\bv_2\|_N
%
\end{align}
%
Using Lemma~\ref{lem:4}, this implies that the following bound holds with high probability for a constant $C$:
%
\begin{align*}
    D_{1,t} 
    &\le C  
    (\|f_t(\bW_t)\|_N+\|f_t(\bV_t)\|_N)^{k-2} \|f_t(\bW_t)-f_t(\bV_t)\|_N\\
    & \le 
    C  (2\|f_t(\bV_t)\|_N+\|f_t(\bW_t) -f_t(\bV_t)\|_N)^{k-2} \|f_t(\bW_t) -f_t(\bV_t)\|_N
    \\
    &\simeq 0.
\end{align*}
%
The last step follows from \eqref{eq:InductionF} and Theorem~\ref{thm:SELAMP}, which implies (recall each $f_{t,s}$ is Lipschitz) that
$\|f_t(\bV_t)\|_N\le C$ with probability $1-o(1)$. Notice that the same argument implies $\|f_t(\bW_t)\|_N \le C$ with high probability.

Similarly, $D_{2,t}\simeq 0$ follows since $\|f_{t_1-1}(\bW_{t_1-1})- f_{t_1-1}(\bV_{t_1-1})\|_N\simeq 0$ and $|d_{t,t_1,k,s}|\le C_T$ by construction, thus yielding \eqref{eq:LAMPapprox1}.


We now prove \eqref{eq:LAMPapprox2}. Comparing \eqref{eq:AMP-def2} and \eqref{eq:LAMP1}, with
$\cP_t^{\parallel} = \bfone-\cP_t^{\perp}$ we find
%
\begin{align}
\label{eq:AMP-LAMP}
    \AMP_{t+1}(\bQ_{t})_k 
    -
    \LAMP_{t+1}(\bQ_{t})_k 
    &= 
    \cP_t^{\parallel} (\bA^{(k)})\{f_t(\bV_t)\}
    -
    \ons_{k,t+1}
    -
    \sum_{0\leq t_1\leq t-1}  
    h_{t,t_1,k}\diamond \qq^{k,t_1+1}\, ,
    \\
\nonumber
    \ons_{k,t+1} 
    &= 
    \sum_{t_1\leq t} 
    d_{t,t_1,k}\diamond f_{t_1-1}(\bV_{t_1-1})
%
\end{align}
%
Note that $\cP_t^{\parallel} (\bA^{(k)})=\E\lt[\bA^{(k)}|\cF_t\rt]$, where $\cF_t$ is the $\sigma$-algebra generated by 
$\{\bq ^{k,s}\}_{t_1\le t, k\le D}$. Equivalently, this is the conditional expectation of $\bA^{(k)}$ given the linear constraints
%
\begin{align}
%
\A^{(k)}\{f_{t_1}(\bV_{t_1})\}&=\by_{k,t_1+1}\, ,\;\;\;\;\;\mbox{ for } t_1\in \{0,\dots, t-1\}\, ,
%
\end{align}
%
Also notice that, by the induction hypothesis, and the definition of $\by_{k,t_1}$, \eqref{eq:Ydef1}, we have for all $t_1\le t$, 
%
\begin{equation}
\label{eq:Y-ons}
    \by_{k,t_1} \simeq  \qq^{k,t_1}+\ons_{k,t_1}\, .
%
\end{equation}
%
Lemma~\ref{lem:symregression} implies that $\cP_t^{\parallel} (\bA^{(k)})$ takes the form of \eqref{eq:SymmRegression} for a suitable matrix
$\hZZ_{k,t}\in\bbR^{N\times t}$. 
The key claim is that
%
\begin{equation}
\label{eq:ZequalsQ}
    \hZZ_{k,t} \simeq \bQ_t\, .
%
\end{equation}
%
In order to establish this claim, we show that,  under the inductive hypothesis,
\begin{equation}
\label{eq:1+TQ=Y}
    (\bfone+\cT_{k,t})\bQ_t\simeq \bY_{k,t}.
\end{equation}
Since $\cL_{k,t}=\bfone +\cT_{k,t}$ is well-conditioned by assumption, the combination of \eqref{eq:ZZ-eq} and \eqref{eq:1+TQ=Y} implies $\hZZ_{k,t}\simeq \bQ_t$. By \eqref{eq:Y-ons}, in order to prove \eqref{eq:1+TQ=Y}, it is sufficient to show that 
\begin{equation}
\label{eq:this-claim}
    \cT_t\bQ_t
    \simeq 
    \ONS_{k,t}
    \equiv 
    [\ons_{k,1}|\cdots|\ons_{k,t}].
\end{equation}

In order to prove \eqref{eq:this-claim}, we use Theorem~\ref{thm:SELAMP}. Recall that 
\begin{align*}
    C_{t_1,t_2,s} &= \E\{U^{k,t_1}_s U^{k,t_2}_s\}\,,
    \\
    W^{t_1}_s &= \sum_{2\leq k\leq D} U^{k,t_1}_s\,,
    \\
    \bC_{\le t} &= (C_{t_1,t_2,s})_{t_1,t_2\le t}\,.
\end{align*}
(The value $2\leq k\leq D$ is implicitly fixed in the definition of $\bC_{\leq t}$.) By Theorem~\ref{thm:SELAMP}, 
\[
    C_{t_1+1,t_2+1} \simeq \<\qq^{k,t_1+1},\qq^{k,t_2+1}\> 
    \simeq 
    (\bG_{\xi^{k,s},t}(\bV))_{t_1,t_2}
    ,
    \quad\forall~t_1,t_2\le t.
\]
This implies for any $0 \le t_1\le t-1$ and $s\in\sS$,
%
\begin{align}
\nonumber
    \sum_{t_2=0}^{t-1}
    (\bG_{\xi^{k,s},t-1}^{-1})_{t_1,t_2}
    R\lt(\qq^{k,t_2+1},f_{t-1}(\VV_{t-1})\rt)_s
    &\simeq 
    \sum_{t_2=0}^{t-1} 
    (\bC_{\le t,s}^{-1})_{t_1+1,t_2+1} 
    \E\lt[
    U^{k,t_2+1}_s f_{t-1,s}(W^0,\dots,W^{t-1})
    \rt] 
    \\
\label{eq:Stein}
    &= 
    \E\lt[
        \frac{\partial f_{t-1,s}}{\partial W^{t_1+1}_s} (W^0_s,\dots,W^{t-1}_s)
    \rt] 
    \bfone_{t_1\le t-2}\, .
%
\end{align}
%
Indeed, Gaussian integration by parts yields the latter expression. Combining \eqref{eq:Stein} with the definition \eqref{eq:AMP-def2} will now allow us to conclude $\cT_{k,t}\bQ_t\simeq \ONS_{k,t}$ as desired. Indeed for each $s\in\sS$ we have
\begin{align*}
    \big[\cT_{k,t}\bQ_t\big]_{t,s} 
    &= 
    \sum_{t_1=0}^{t-1} 
    (\bGG_{\xi^{k,s},t-1})_{t_1,t-1} 
    \f_{t_1,s}
    \Big(
    \sum_{t_2=0}^{t-1} 
    (\bG_{\xi^{k,s},t-1}^{-1})_{t_1,t_2} 
    \,
    R_s(\qq^{k,t_2+1}, \f_{t-1})
    \Big)
    \\
    &\simeq 
    \sum_{t_1=0}^{t-2}
    \zeta^{k,s}
    \big(
    \vR(\f_{t_1}, \f_{t-1})
    \big)
    \f_{t_1,s}
    \cdot 
    \E\lt[
    \frac{\partial f_{t-1,s}}{\partial W^{t_1+1}_s} 
    (W^0_s,\dots,W^{t-1}_s)
    \rt]
    \\
    &= 
    \ons_{k,t}.
\end{align*}
Having established \eqref{eq:ZequalsQ}, we now use the formula \eqref{eq:SymmRegression} for $\cP^{\parallel}_t(\bA^{(k)})=\E\big[\bA^{(k)}|\cF_t\big]$. The result is:
%
\begin{align}
\label{eq:AParallel}
    \cP^{\parallel}_{t}(\bA^{(k)})\{\f_t\}
    &\simeq 
    \sum_{t_1\leq t}
    \big(\alpha_{t_1}
    \diamond
    \qq^{k,t_1}
    +
    \beta_{t_1}
    \diamond
    \f_{t_1}\big)\, ;
    \\
\nonumber
     \alpha_{t_1,s}
     &= 
     \sum_{0\leq t_2\le t-1} 
     (\bG_{\xi^{k,s},t-1}^{-1})_{t_1,t_2} 
     \,
     \xi^{k,s}\big(
     \vR(
     f_{t_2}(\VV_{t_2}),f_{t}(\VV_t)
     )
     \big)
     \, ,
     \\
\nonumber
    \beta_{t_1,s} 
    &= 
    \Big(
    \sum_{0\le t_2\leq t-1} 
    (\bG_{\xi^{k,s},t-1}^{-1})_{t_1,t_2} 
    \,
    R_s( \qq^{k,t_2},\f_{t} )
    \Big) 
    \zeta^{k,s}\big(
    \vR( \f_{t_1},\f_{t} )
    \big).
%
\end{align}
On the other hand, using again \eqref{eq:Stein} gives
%
\begin{align*}
    \sum_{t_1\leq t}\beta_{t_1}\diamond \f_{t_1} 
    &\simeq  
    \sum_{t_1 \le t-1}  d_{t,t_1,k}\diamond \f_{t_1-1}  
    =
    \ons_{k,t+1},
\\
    \sum_{t_1\leq t}
    \alpha_{t_1}
    \diamond
    \qq^{k,t_1} 
    &\simeq 
    \sum_{0\leq t_1\leq t-1}  
    h_{t,t_1,k}
    \diamond
    \qq^{k,t_1+1}.
\end{align*}
%
We conclude from \eqref{eq:AMP-LAMP} that $\|\AMP_{t+1}(\bQ_{t})_k -\LAMP_{t+1}(\bQ_{t})_k  \|_N\simeq 0$. This concludes the proof.
\end{proof}


